Space-time large deviations in capacity-constrained relay networks

We consider a single-cell network of random transmitters and fixed relays in a bounded domain of Euclidean space. The transmitters arrive over time and select one relay according to a spatially inhomogeneous preference kernel. Once a transmitter is connected to a relay, the connection remains and the relay is occupied. If an occupied relay is selected by another transmitters with later arrival time, this transmitter becomes frustrated. We derive a large deviation principle for the space-time evolution of frustrated transmitters in the high-density regime.

==> Intro.tex <==
\subsection{Definition of the dynamic network model}
\label{modDefSec}
We consider a Poisson point process of users in a bounded domain $\vW\subset\R^d$ who want to transmit data to a basestation located at the origin. Data will transmitted in an time interval $[0,T]$. Further we assume that the data bandwidth that is required by every user is independent of the other users and has values in $\{0,1\}$. More formally, the bandwidth requirement over time is an element of the space ${\vD}$ of functions $\phi:\,[0,T]\to\{0,1\}$ which have only finitely many jumps.
%represents the bandwidth requirement of the user under consideration. 
Let $\mu$ denote the intensity measure of the combined point process of the spatial user distribution together with their $iid$ marks distributed on ${\bf{N}}$. The Poisson point process with intensity measure $\mu$ on $\vW\times\bf{N}$ we denote by $\vX$.

\medskip
Users will have the possibility to transmit their data either directly to the base station or via one other user who acts as a relay. In particular the use of relaying extends the transmission range as wvell as the capacity of the network. 
The data rate each user can transmit over a certain distance $r$ is assumed to be bounded by $\vell(r)$ where $\vell:\vW^2\to[0,1]$ is a decreasing function. For instants a user $\vX_i$ can always transmit $\vell(|\vX_i-x|)$ to a spatial location $x\in \vW$ and 
$$\min\{1-\vell(\vX_i,o),\vell(\vX_i,x)\}$$
represents the required relay capacity at position $x$ taking into account the upper bound given by the distance between $\vX_i$ and $x$.
Moreover, the effective amount of data that can be transmitted depends additionally on the capacity available at the relay, i.e., 
$$\bw(\vX_i,x,b)=\min\{1-\vell(\vX_i,o),\vell(\vX_i,o),\vell(x,o)-b\}$$
where $b>0$ represents the current traffic through the relay $x$. Moreover, for convenience, we put $\bw(\vX_i,\vdag,b)=0$.
In the following we construct a dynamic network model where the routing decision of a user is based on the available capacities of the other users. The capacity itself depends on previous routing decisions made in the network. Let us assume for convenience, that at time $t=0$ all users have $0$ status and therefore do not transmit. In order to describe the network model, we associate to each user $\vX_i$ three quantities $\vB_t(\vX_i)$,  and $\vR_t(\vX_i)$. We first provide a general description of these quantities and then move to precise mathematical definitions.

First, $\vR_t(\vX_i)\in\{\vdag\}\cup \vX$ denotes the \emph{relay node used by transmitter $\vX_i$ at time $t>0$}. Once a relay is chosen by $\vX_i$, this choice remains fixed for a non-trivial time interval, so that $\vR_t(\vX_i)$ jumps only at finitely many points in time. These jumps are triggered by the following events.
\begin{enumerate}
	\item {\bf Start of transmission.} If $t$ is such that $\vX_i(t)=1$ and $\vX_i(t-)=0$, then the $i$th user starts sending data at time $t$. If $\vX_i$ is close to the base station, then it might be possible that data can be transmitted to the base station at the required rate directly. In this case, no relay is needed. However, typically the direct connection is only sufficiently strong to sustain traffic at a smaller rate, so that the remaining traffic needs to be offloaded through relaying. We assume that in this case the choice of relay is probabilistic, where relay nodes that are able to offer a higher bandwidth are chosen more likely.
	\item {\bf End of transmission.} If $t$ is such that $\vX_i(t)=0$ and $\vX_i(t-)=1$, then the $i$th user stops sending data at time $t$. In particular, there is no longer need for relaying and we put $\vX_i(t)=\vdag$.
	\item {\bf Breakdown of relay.} Let $\vX_j=\vR_t(\vX_i)$ the relay associated with the $i$th user at time $t$. If $t$ is such that $\vX_j(t)=1$ and $\vX_j(t-)=0$, then the $j$th user wants to start sending data at time $t$. We assume that $\vX_j$ is willing to offer relay services to other users during idle time, but when she needs to transmit data herself relaying is no longer tolerated and all users relaying via $\vX_j$ have to find different routing nodes.
\end{enumerate}

One of the most important features of our network model is the possibility to represent traffic congestions, when too many transmitters try to use a single relay at the same time. For this purpose, we also need to track the \emph{relay traffic $\vB_t(\vX_i)\ge0$ at the node $\vX_i$ at time $t>0$}. If the node $\vX_i$ is acting as a \emph{relay}, this traffic is simply the data rate of the transmission of the base station. As mentioned before, the maximum bandwidth decreases with distance to the base station and is bounded above by $\vell(\vX_i,o)$. Additionally, the bandwidth decreases further with every transmitter using $\vX_i$ as relay. On the other hand, if $\vX_i$ is acting as \emph{transmitter}, then relay traffic is to be understood as the rate at which data is sent to the relaying node. Again, the maximum bandwidth never exceeds $\vell(\vX_i-\vX_j|)$, but can be even smaller if there is not enough free capacity at $\vX_j$.
Similarly to $\vR_t(\vX_i)$, changes in the traffic $\vB_t(\vX_i)$ are triggered by the occurrence of certain events.
\begin{enumerate}
	\item {\bf Start of transmisson.} If $t$ is such that $\vX_i(t)=1$ and $\vX_i(t-)=0$, then the $i$th user starts transmitting data at time $t>0$. Let $\vX_j$ denote the relay chosen by $\vX_i$ at time $t$, i.e., $\vR_t(\vX_i)=\vX_j$. Before accepting traffic from $\vX_i$ the user $\vX_j$ already has to handle traffic at rate $\vB_{t-}(\vX_j)$. Hence, at $\vX_j$ the amount of spare capacity for further relay traffic is given by $\vell(|\vX_j|)-\vB_{t-}(\vX_j)$ and we put $\vB_t(\vX_i)=\bw(\vX_i,\vX_j,\vB_{t-}(\vX_j))$.
	\item {\bf End of transmission.} If $t$ is such that $\vX_i(t)=0$ and $\vX_i(t-)=1$, then the $i$th user stops transmitting data at time $t>0$. Since relay traffic is only initiated if transmitting nodes look for relay possibilities, there will be no relay traffic through $\vX_i$ at time $t$, i.e., $\vB_t(\vX_i)=0$.
	\item{\bf Breakdown of relay.} If just before time $t$ the $i$th user relays via $\vX_j$ and if $\vX_j$ starts transmitting data at time $t$, then $\vX_j$ is no longer available as relay to $\vX_i$. Therefore, $\vX_i$ has to choose a new relay and the relay traffic is computed using the same formula as in the case of a transmission start.
	\item {\bf Change of relay traffic.} Assume that $\vX_j$ starts transmitting data at time $t$ and chooses $\vX_i$ as a relay, i.e., $\vX_j(t)=1$, $\vX_j(t-)=0$ and $\vR_t(\vX_j)=\vX_i$. Then, the relay traffic at $\vX_i$ is increased by the size of the relay traffic originating at $\vX_i$, i.e., 
		$$\vB_t(\vX_i)=\vB_{t-}(\vX_i)+\bw(\vX_j,\vX_i,\vB_{t-}(\vX_i)).$$
	A similar effect appears if at time $t$ some transmitter using $\vX_i$ as relay stops sending. 
\end{enumerate}

After this discussion, we now provide precise definitions of the quantities $\vB_t(\vX_i)$ and $\vR_t(\vX_i)$. Since both $\vB_t(\vX_i)$ and $\vR_t(\vX_i)$ change only at discrete points in time, they can be defined recursively. We start by putting $\vB_0(\vX_i)=0$ and $\vR_0(\vX_i)=\vdag$ for all $\vX_i\in \vX$. In the recursion, the definitions of $\vB_t(\vX_i)$ and $\vR_t(\vX_i)$ make use of the quantities $\vB_{t-}(\vX_j)$ and $\vB_{t-}(\vX_j)$ for arbitrary $\vX_j\in \vX$. Moreover, the definition of $\vB_t(\vX_i)$ may involve $\vR_t(\vX_i)$, but not vice versa. Making the loose descriptions provided above formal, we define $\vB_{t}(\vX_i)$ via
$$
\vB_t(\vX_i)=\begin{cases}
	\bw(\vX_i,\vR_t(\vX_i),\vB_{t-}(\vR_t(\vX_i)))&\text{if $\vR_{t-}(\vX_i)\ne \vR_t(\vX_i)$}\\
	\vB_{t-}(\vX_i)-\bw(\vX_j,\vX_i,\vB_{t-}(\vX_i))&\text{if $\vX_i=\vR_{t-}(\vX_j)\ne \vR_{t}(\vX_j)$ for some $\vX_j$},\\
	\vB_{t-}(\vX_i)+\bw(\vX_j,\vX_i,\vB_{t-}(\vX_i))&\text{if $\vX_i=\vR_t(\vX_j)\ne \vR_{t-}(\vX_j)$ for some $\vX_j$},\\
	\vB_{t-}(\vX_i)&\text{otherwise}.
\end{cases}
$$
Next, we deal with the definition of the relay choices $\vR_t(\vX_i)$, recalling from our above remarks that these choices involve additional randomness. More precisely, we assume that there exists a kernel function $f$ such that conditioned on $\vX$ and $\{(\vX_j,\vB_{t-}(\vX_j))\}_{j\ge1}$ the probability that $\vR_t(\vX_i)$ equals $x\in \{\vdag\}\cup \vX$ is given by 
$$\vk(x,\vX_i,\vX,\{(\vX_j,\vB_{t-}(\vX_j))\}).$$
We assume that 
$$\vk(\vX_j,\vX_i,\vX,\{(\vX_j,\vB_{t-}(\vX_j))\})=0$$
if $\vell(|\vX_j|)=\vB_{t-}(\vX_j)$, that is if the node $\vX_j$ is already saturated. {\bf Add further conditions and an example for $\vk$}.

Making use of the kernel function $\vk$, the dynamics of $\vR_t(\vX_i)$ is defined as follows.
$$
\vR_t(\vX_i)=
\begin{cases}
	\vdag&\text{if $\Delta \vX_i(t)=-1$},\\
	Z&\text{where $Z\sim \vk(\vX_i,\cdot,\{\vX_j,\vB_{t-}(\vX_j)\}_j)$ if $\Delta \vX_i(t)=1$ or $\Delta(\vR_{t-}(\vX_i))(t) =1$},\\
	\vR_{t-}(\vX_i)&\text{otherwise}.
\end{cases}
$$
In particular, conditioned on $\vX$ the process $\{\{(R_{t}(X_i),B_t(X_i)\}_{X_i\in X}\}_{0\le t\le T}$ is Markovian in time.

\subsection{Major issue: definition of dynamic network model for arbitrary measures}
{\bf What is the correct state space when passing to the high-density limit? Is it possible to stay in the world of level 2?}

\subsection{Definition of frustration}
The main result of this paper is a large-deviation analysis of frustration events related to traffic congestions at certain relay nodes. In order to define such frustration events, we first introduce an empirical measure of $\vtau$-frustrated users, which can be used to define a large variety of frustration events. In order to understand the high-density limit $\lambda\to\infty$, it is important to perform a transition from pure point measures to absolutely continuous measures. In order to define an analog of the empirical measure of $\vtau$-frustrated users in the absolutely continuous setting, some preparatory steps are needed.
\subsubsection{Definition for point processes}
Let 
$$\vBp_t(X_i)=
\begin{cases}
	0	&\text{if $\vX_i(t)=0$},\\
	1-(\vell(\vX_i)+\vB_t(\vX_i))&\text{if $\vX_i(t)=1$}\\
\end{cases}$$
denote the \emph{bandwidth gap} that user $\vX_i$ experiences at time $t>0$. The amount of frustration caused by unmet bandwidth demands that the $i$th user experiences will be encoded as $\vtau(\{\vBp_t(X_i)\}_{0\le t\le T})$ for some measurable and decreasing function $\vtau:[0,1]^{[0,T]}\to[0,\infty)$. The principal object of investigation in this paper is the empirical measure $\vL_\lambda[\vtau]$ of $\vtau$-frustrated users given by 
	$$\vL_\lambda[\vtau]=\frac1\lambda\sum_{\vX_i\in\vX^\lambda}\vtau(\vBp_t(\vX_i))\delta_{\vX_i}.$$
When considering 

\subsubsection{Definition for general measures}
Next, we define an analog of the empirical measure $\vtau$-frustrated users for general measures. First, it is important to identify the correct space where these measures should be defined. A first attempt could be to use finite measures on the space $\vW\times\vD$ that would allow to encode distributions involving both the spatial location of users as well as the data-traffic evolution in time. However, recalling the dynamics of relay choices explained in Section~\ref{modDefSec}, we observe that there is additional randomness involved every time a transmitter needs to choose a relay. This additional randomness cannot be neglected when performing a large deviation analysis and therefore we consider finite Borel measures on the space 
$$\vPi=\vW\times\vD\times\N^{[0,T]},$$
where the third component gives for each time point in $[0,T]$ the index of the relay chosen at this time. 


==> LDPDiscrete.tex <==
\subsection{Large deviations for the upper bound}
%In order to prove the continuity of $\b$, we need to show that the solutions of~\eqref{DE_Cont} depend continuously on the input measure $\nu$. 
First, we show that the solution map $\nu\mapsto\b(\nu)$ is continuous at every $\nu\in\MM_{\ms{ac}}$. This continuity is the crucial step in the proof of the upper bound in Proposition~\ref{LDP_NoSpatial}, as it will allow us to apply the contraction principle~\cite[Theorem 4.2.1]{dz98}.

\begin{proposition}
	\label{mapContLem}
	Let $\nu\in\MM_{\ms{ac}}$ be arbitrary. Then, the map $\nu\mapsto\b(\nu)$ restricted to $\MM_\mu$ is continuous at $\nu$.
\end{proposition}
Next we prove a Sanov-type LDP for the empirical distribution.
\begin{proposition}\label{SanovDiscrete}
The random measures $L^\la_{\ms{T},\bf y}$ satisfy a LDP in the projective-limit topology with good rate function given by
$$I(\nu)=h(\nu|\mu_{\ms{T},{\bf y}}).$$
\end{proposition}
Using this proposition, the proof of the upper bound in Proposition~\ref{condLDPProp} is essentially an application of the continuity of solutions, whenever they exist, w.r.t.~the driving measure.  
\begin{proof}[Proof of upper bound in Proposition~\ref{condLDPProp}]
	Let $F$ be upper semicontinuous. Then, by Proposition~\ref{SanovDiscrete},
	\begin{align*}
		\limsup_{\la\to\infty}\la^{-1}\log\E\exp(\la F(\g(L_\la)))&= \limsup_{\la\to\infty}\la^{-1}\log\E[\one\{L_\la\in \MM_o\}\exp(\la F(\g(L_\la)))]\\
									  &\le-\inf_{\nu\in\MM}\{h(\nu|\mu)-G(\nu)\},
	\end{align*}
	where $G:\MM\to[0,\infty)$ is the upper semicontinuous regularization of the map 
	$$\nu\mapsto -\infty\one\{\nu\not\in \MM_o\}+F(\g(\nu)).$$
	It remains to show that for every $\nu\in\MM_{\ms{ac}}$, we have that $G(\nu)\le F(\g(\nu))$. Indeed, in Proposition~\ref{mapContLem} we have seen that $\g(\nu')$ becomes arbitrarily close to $\g(\nu)$ if $\nu'\in\MM_o$ is sufficiently close to $\nu$. Therefore, using the upper semicontinuity of $F$ concludes the proof.
	\end{proof}

\subsection{Large deviations for the lower bound}
For the lower bound, we follow a different and unfortunately more technical and more restrictive line of arguments then for the upper bound. The main reason why we can not follow the same steps is that existence of solution can not be guaranteed away from measures which are either absolutely continuous or purely atomic. Here we construct trajectories via an Euler-type scheme which are lower approximations to the lower extremal solutions of the squared integral operator which always exist. These approximations are constructed via a local one-step Piccard iteration which uses an Euler approximation as input. The resulting trajectories are continuous-time and exhibit good continuity properties w.r.t.~driving measures. In the present section, we first provide precise definitions of the approximations and show that they satisfy large-deviation principles.

Let $\de>0$ and consider the discretization of $[0,T]$ into $T/\de$ disjoint segments of length $\de$. 
To define the approximation, we proceed recursively and start by putting $\bdde_0=0$. Once $\bdde_{(n-1)\de}$ is available, we define the locally constant function
\begin{align*}
	\bddde_{t}=\bdde_{(n-1)\de}+\nu_{\ms{T}}\big(((n-1)\de,n\de]\times[0,1]\big)
\end{align*}
for $t\in((n-1)\de,n\de]$. {\bf Note that here, we count also the arrival of users in outage.}
Then,  for $t\in((n-1)\de,n\de]$ we put 
\begin{align*}
	\bdde_{t}=\bdde_{(n-1)\de}+\nu_{\ms{TU}}\big(((n-1)\de,t]\times[r^{-1}\bddde_{n\de}(W),1]\big).
\end{align*}
In case $\nu_{\ms{R}}=0$ we set $\bdde=0$. 
We can think of $\bddde$ as a discretized approximation of the operator $\mc{T}$ applied once to the zero function. Similarly, $\bdde$ corresponds to an approximation of $\mc{T}^2$ applied to the zero function. 
Note that if $\nu$ is atomless, then the trajectorie $\bdde$ is continuous w.r.t.~time.

\medskip
We can now introduce the approximating process of frustrated users by setting 
$$\gdde_t(\nu)=\nu_{\ms{T}}([0,t]\times[0,1]\times\{\ms{O,U}\})-\bdde_t(\nu)$$
and establish comparison results w.r.t~the actual process of frustrated user $\g$. 





In order to obtain the lower bound in the LDP for the approximating trajectories of busy users we apply the contraction principle to the LDP given in Proposition~\ref{SanovDiscrete}. This is possible since the trajectories $\bdde$ depend continuously on the driving measure $\nu$ at least for those $\nu$ which do not have infinite relative entropy w.r.t.~$\mu$. This is what we show now.

\begin{lemma}\label{ContractionDiscrete}
The mappings $\MM\to\LL$ given by $\nu\mapsto\bdde(\nu)$ is continuous w.r.t.~the projective-limit topology and the topology of point-wise convergence at any $\nu\in\MM_{\ms{ac}}$.
\end{lemma}

\begin{corollary}
The random process $(\la^{-1}B^{\de}_t)_{0\le t\le T}$  satisfies a LDP with good rate functions given by
$$I^{D}(b)=\inf_{\nu:\,\bdde(\nu)=b}h(\nu|\mu).$$
\end{corollary}



==> OutlineProof.tex <==
\section{Outline of proofs}
\label{outlineSec}
As a first attempt it would be natural to use a Sanov-type result for the user distribution $\nu$ and apply the contraction principle for solutions of the associated differential equation. The main part of the proof would be to show continuity of solutions w.r.t.~the user distribution. However, for general measures $\nu$ already the existence of solutions is violated. 
Therefore we choose a different route and consider a time-discretized Euler scheme for the original process. 
First we show that some monotonically approximating discrete-time solutions of this scheme depend continuously on $\nu$. Using this together with Sanov's theorem gives a large deviation principle for the time-discrete process. After slight modifications of the driving measure, solutions of the discretized process can be bounded from above and from below by the extremal fixed points of the squared integral operator. Together with the increasingness assumption on the observables $F$ this will establish the desired inequalities. 
%After that we show that solutions for increasingly fine discretizations form an exponentially good approximation for the continuous-time process. After identification of the rate function we obtain both existence and uniqueness of solutions and the large deviation principle stated in Theorem~\ref{LDP_NoSpatial}.
The idea for the modifications is to increase transmitters in certain regions in such a way that dominance relations between the trajectories hold, while the cost of the modifications negligible on the exponential scale. 

\subsection{Discretized relay locations}
TBA
\subsection{Discretized transmitter locations}
TBA

\subsection{Large deviations in the spatially discretized case}
In order to derive the results in Theorem~\ref{LDP_NoSpatial} and Theorem~\ref{LDP_Spatial} we will first work on an intermediate setting, where the there is a spatial component, but only finitely many spatial regions are considered. Theorem~\ref{LDP_NoSpatial} will then be a simple corollary where there is only a single spatial component. Additionally, for the proof of Theorem~\ref{LDP_Spatial}, we build on this result and use a limiting procedure where the spatial discretization tends to the continuum. 
%More precisely, assume that $\k$ and $p$ are of the form \eqref{Abflachung} for a spatial discretization $W_1,\dots, W_k$ of $W$, then $(\mu(l_{\ms R}^\la),l_{\ms R}^\la)$ is locally constant. We will be interested in the joint evolution of
%\begin{align*}
%\g_t{(\nn,\nu_{\ms R})}(W_i,W_j)=\nn([0,t],[0,1],\{\ms{O,U}\},W_i, W_j)-\bb_t(\nn,\nu_{\ms R})(W_i, W_j)
%\end{align*}
%for $1\le i,j\le k$.

%\bigskip
%In order to treat inhomogeneous probability kernels $\k$, as given in equation \eqref{Kappa}, we perform a limiting procedure w.r.t.~discretizations of $W$. 
%In this subsection we perform the first step into this direction by introducing a finite discretization of $W$ and tracking the transmitter locations in this discretization.
%More precisely, 
%%First note that, conditioned on a realization of relays $X^\la_{\ms R}$, the process of transmitters $X_{\ms{T},X^\la_{\ms R}}^{\lambda}=\{(T_i,U_i,X_i,Y_i,\s_{\ms{O}})\}_{i\ge1}$ which connect to possible relay locations $Y_i\in X^\la_{\ms R}$ has intensity measure
%%$$\la\a(\mu_{\ms T},L^\la_{{\ms R}})(\d t, \d u, \d x,\d y,\d \s_{\ms{O}})=\la\frac{\k(x,y)}{\int \k(x,y)L^\la_{{\ms R}}(\d y)}(\mu_{\ms T}\otimes L^\la_{\ms R})(\d t,\d u,\d x,\d y,\d \s_{\ms{O}}).$$
%%%
%%%Let $W^\delta$ be a sequence of partitions where every subdomain is connected and its volume is smaller then $\delta>0$. 
%let ${\bf x}=(x_i)_{0\le i\le n}$ be a finite set of center-points of a discretization $W_i=W(x_i)$ of $W$. 
%%where $\sup_{x_i\in\bf x^\de}\text{diam}(W^\de(x_i))<\de$. 
%Let 
%$$\bar\mu^\de_{\ms T}=P\otimes U\otimes\ms{Ber}_{p_{\ms{O}}}\otimes\mu^\de_{\ms T}$$ 
%where $\mu^\de_{\ms T}$ is a measure on $\{W^\de(x_i):\, x_i\in\bf x^\de\}$.

\begin{proposition}\label{LDP_DiscSpatial}
Let $\k$ and $p$ are of the form~\eqref{Abflachung} for a spatial discretization $w=(W_1,\dots, W_k)$ of $W$. Let $F:\,\LL'\to[-\infty,\infty)$ be a bounded function which is discretized w.r.t.~$w$. 
If $F$ is upper semicontinuous in the $\tau$-topology, then 
\begin{align*}
\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp[\la F(\G^\la)]\le -\inf_{\nn\in\MM_{\ms {lc}}}\{h(\nn|\mu(\mu_{\ms R}))-F(\g(\nn,\mu_{\ms R}))\}
\end{align*}
and if $F$ is lower semicontinuous in the $\tau$-topology, then
\begin{align*}
\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp[\la F(\G^\la)]\ge -\inf_{\nn\in\MM_{\ms {lc}}}\{h(\nn|\mu(\mu_{\ms R}))-F(\g(\nn,\mu_{\ms R}))\}.
\end{align*}
\end{proposition}
The proof for the upper bound in Proposition~\ref{LDP_DiscSpatial} is based on the contraction principle and Sanov's theorem. In particular, we will establish existence and continuity properties of the path of frustrated users w.r.t.~absolutely continuous driving measures using Schauder's fix point theorem and monotonicity arguments.

The lower bound is more involved because also non-absolutely continuous measures have to be taken into account. Here, existence of solutions can not be guaranteed and therefore the contraction principle can not be applied directly. Our approach will be to condition on a non-spatial setting, which will be considered first. The main ingredient is to consider an approximating process and show that this approximation is close to the original process with high probability using coupling methods. We then derive the following intermediate result for which we need to introduce notation. For a time-discretization of $[0,\TF]$ write 
$$\Delta_j \G^\la(W_i\times W_{i'})=\G^\la_{t_j}(W_i\times W'_{i'})-\G^\la_{t_{j-1}}(W_i\times W'_{i'}).$$
Moreover, let 
$$\mathbb{S}_{k_x}^{k_yk_T}=\{(u_{i,i',j})_{i,i',j}\in[0,1]^{k_xk_yk_T}:\,\sum_{i=1}^{k_x}u_{i,i',j}=1\}$$
denote the product of $k_yk_T$ simplices in $[0,1]^k_x$.
For ${\bf u}\in \mathbb{S}_{k_x}^{k_yk_T}$ we let ${\bf u}\circ \gamma$ denote the trajectory defined by
$$({\bf u}\circ \gamma)_{t_j}(W_i\times W_{i'})=\sum_{j'=1}^j u_{i,i',j'}\Delta_{j'}\gamma(W\times W_{i'}).$$
\begin{proposition}
        \label{condLDPProp2}
        Let $F:\,\LL'\to[-\infty,\infty)$ be a measurable, bounded and increasing function. 
        If $F$ is lower semicontinuous in the $\tau$-topology, then
        \begin{align*}
		\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp[\la F(\G^\la)]	&\ge -\inf_{\nu\in \mathcal{M}}[h(\nu|\bar\mu_{\ms T})-F^*(\g(\nu)(W\times\cdot))].,
        \end{align*}
	where
	$$F^*(\g)=\sup_{{\bf u}\in\mathbb{S}^{k_yk_T}_{k_x}}\big\{F({\bf u}\circ {\g})-\sum_{i'=1}^{k_y}\sum_{j=1}^{k_T}\Delta_j\g(W\times W_{i'}')h({\bf u_{\cdot,i',j}}|{\bf p}) \big\}.$$
        \end{proposition}
As a second step, we will identify the rate function on the r.h.s.~of Proposition~\ref{condLDPProp2} with the desired rate function of Proposition~\ref{LDP_DiscSpatial}.

\begin{proposition}
        \label{condLDPProp3}
        Let $F:\,\LL\to[-\infty,\infty)$ be a measurable and bounded function, then
        %If $F$ is lower semicontinuous in the $\tau$-topology, then
        \begin{align*}
\inf_{\nu\in \mathcal{M}}[h(\nu|\bar\mu_{\ms T})-F^*(\g(\nu)(W\times\cdot))]		&=\inf_{\nu\in\mathcal{M}}\{h(\nu|\bar\mu_{\ms T})-F(\g(\nu))\}.
        \end{align*}
\end{proposition}

\begin{proof}[Proof of Proposition~\ref{condLDPProp3}]
We first prove
\begin{align*}
\sup_{\nu\in \mathcal{M}'}[F^*(\g(\nu)(W))-h(\nu|\bar\mu_{\ms T})]		&\ge\sup_{\nu\in\mathcal{M}}\{F(\g(\nu))-h(\nu|\bar\mu_{\ms T})\}.
        \end{align*}
Let $\nu\in\MM$, then it suffices to construct $\nu'$ and ${\bf u}$ such that 
\begin{align*}
F({\bf u}\circ {\g(\nu')})-\sum_{j=1}^{k_T}\Delta_j\g(\nu')(W)h({\bf u_{\cdot,i',j}}|{\bf p})-h(\nu'|\bar\mu_{\ms T})&\ge F(\g(\nu))-h(\nu|\bar\mu_{\ms T}).
        \end{align*}
Setting $\nu'(\d t,\d u,\d\s)=\nu(W,\d t,\d u,\d\s)$ and $u_{i,i',j}=\frac{\Delta_j\g(\nu)(W_i\times W)}{\Delta_j\g(\nu')(W)}$, we have that ${\bf u}\circ {\g(\nu')}=\g(\nu)$ and the terms involving $F$ cancel out. Further note that 
\begin{align*}
h(\nu|\bar\mu_{\ms T})=h(\nu'|\bar\mu_{\ms T})+\int\d\nu' h({\bf q}|{\bf p})
\end{align*}   
where $q_i=\frac{\d\nu(W_i)}{\d\nu'}(t,u,\s)$ and hence it suffices to show that
\begin{align*}
\Delta_j\g(\nu')(W)h({\bf u_{\cdot,j}}|{\bf p})\le \int_{t_{j-1}}^{t_j}\d\nu' h({\bf q}|{\bf p})
\end{align*}
for all $1\le j\le k_T$. Now, $\Delta_j\g(\nu')(W_i\times W)=\int_{A_{j}}\d\nu(W_i)$ where 
$$A_{j}=\{(s,u,\s):t_{j-1}\le s\le t_j, 0\le u\le \b_s(\nu')(W),\s=\ms U\}\cup\{(s,u,\s):t_{j-1}\le s\le t_j, \s=\ms O\}$$ and in particular, it suffices to show that  
\begin{align*}
\int_{A_{j}}\d\nu'h({\bf u_{\cdot,j}}|{\bf p})\le \int_{A_{j}}\d\nu' h({\bf q}|{\bf p})
\end{align*}   
for all $1\le j\le k_T$ since $h\ge 0$. But  
\begin{align*}
\sum_i\int_{A_{j}}\d\nu' q_i\log\frac{q_i}{p_i}&=\sum_i\int_{A_{j}}\d\nu' q_i[\log\frac{u_{i,j}}{p_i}+\log\frac{q_i}{u_{i,j}}]\cr
&=\int_{A_{j}}\d\nu'h({\bf u_{\cdot,i',j}}|{\bf p})+\int_{A_{j}}\d\nu' h({\bf q}|{\bf u}_{\cdot,j})
\end{align*}   
and $\int_{A_{j}}\d\nu' h({\bf q}|{\bf u}_{\cdot,j})\ge 0$ as required.   
        
For the other inequality, let $\nu'$ and ${\bf u}$ be arbitrary and define $\nu$ via $\frac{\d\nu(W_i)}{\d\nu'}1_{A_j}=u_{i,j}$ and $\frac{\d\nu(W_i)}{\d\bar\mu_t}1_{A^c_j}=1$, then,
\begin{align*}
({\bf u}\circ {\g(\nu')})_{t_j}(W_i\times W)&=\sum_{j'=1}^j u_{i,j'}\Delta_{j'}\gamma(\nu')(W)=\sum_{j'=1}^j \int_{A_{j'}}\d\nu' u_{i,j'}\cr
&=\sum_{j'=1}^j \int_{A_{j'}}\d\nu(W_i)=\sum_{j'=1}^j \Delta_{j'}\gamma(\nu)(W_i)=\gamma(\nu)_{t_j}(W_i)
\end{align*} 
and thus again it suffices to verify that 
\begin{align*}
\sum_{j=1}^{k_T}\Delta_j\g(\nu')(W)h({\bf u_{\cdot,j}}|{\bf p})+h(\nu'|\bar\mu_{\ms T})&\ge h(\nu|\bar\mu_{\ms T}).
\end{align*}
Note that, in the entropy, by the definition of $\nu$, the integration domain is just $\cup_{j}A_j$ and thus
\begin{align*}
h(\nu|\bar\mu_{\ms T})=h(\nu'|\bar\mu_{\ms T})+\sum_{j=1}^{k_T}\int_{A_j}\d\nu' h({\bf u_{\cdot, j}}|{\bf p}).
\end{align*} 
But $\int_{A_j}\d\nu' =\Delta_j\g(\nu')(W)$ which finishes the proof.    
\end{proof}


%\subsection{Supporting result for the proof of Theorem~\ref{LDP_Spatial}}
%
%
%\subsection{Old stuff}
%For the proof of Theorem~\ref{LDP_NoSpatial} it is convenient to first condition on the number of relays and derive an LDP where the number tends to infinity linearly in $\lambda>0$. As a corresponding result will also be important for the proof of the more general Theorem~\ref{LDP_Spatial}, we state this conditioned LDP in a setting involving also locations of the relays. More precisely, consider a set ${\bf{y}}=\{y_1,\dots,y_k\}$ of sites in $W$ and assume relays of masses ${\bf r }=\{r_1,\dots,r_k\}$ to be positioned on ${\bf{y}}$. We denote by $l_{\bf y,r}=\sum_{i=1}^kr_{i}\de_{y_i}$
%the empirical measure of relays where $\bf r$ can either be deterministic or given by random variables $R_{\la, i}=S_i/\la$ where $S_i$ are independent Poisson distributed with intensities $\la\mu_{\ms R,i}$. 
%
%The form of the rate function can be intuitively understood as follows. In a two-step procedure, we first condition on the number of relays in each location in $\bf y$, represented by the $k$-vector $\bf r$. 
%A major part of the work will be dedicated to the proof of the following proposition. Here the number of relays at the locations $\bf y$ is assumed to be fixed and the optimization is purely w.r.t.~transmitters. 
%
%\bigskip
%For the proof of Theorem~\ref{LDP_SpatialDiscr} define $p_i=\mu_{\ms T}(W^\de_i)/\mu_{\ms T}(W)$.
%
%
%
%
%\begin{proposition}
%        \label{condLDPProp}
%        Let $F:\,\LL\to[-\infty,\infty)$ be a measurable, bounded and increasing function. If $F$ is upper semicontinuous in the $\tau$-topology, then
%        \begin{align*}
%		\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp[\la F(\g(L^\la_{\ms{T},\bf y},l_{\bf y,r}))]\le -\inf_{\nu\in\MM_{\ms {lc}}}\{h(\nu|\mu(l_{\bf y,r}))-F(\g(\nu,l_{\bf y,r}))\}
%        \end{align*}
%        and if $F$ is lower semicontinuous in the $\tau$-topology, then
%        \begin{align*}
%		\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp[\la F(\g(L^\la_{\ms{T},\bf y},l_{\bf y,r}))]\ge -\inf_{\nu\in\MM_{\ms {lc}}}\{h(\nu|\mu(l_{\bf y,r}))-F(\g(\nu,l_{\bf y,r}))\}.
%        \end{align*}
%        \end{proposition}
%%In the above proposition, the number of relays in the system is assumed to be adapted to the limiting procedure but deterministic. 
%%In the following proposition, the number of relays, still positioned at non-random locations $\bf y$, will be assumed to be Poisson distributed. This leads to the appearance of an additional term in the entropic part of the rate function. More precisely, let $R_i$ be independent and Poisson distributed random variables with intensities $\la\mu_{\ms R}(y_i)$ and denote $L^\la_{\bf y}=\la^{-1}\sum_{i=1}^kR_i\de_{y_i}$.
%%%the relays are now assumed to form a Poisson point process with intensity $\mu_{\ms R}$ and $\bs \mu_{\ms R,{\bf W}}=(\mu_{\ms R}(W_1),\dots,\mu_{\ms R}(W_k))$.
%For the proof of Theorem~\ref{LDP_Spatial} we will consider the case where the spatial discretization tends to the continuum, using smoothness of the connection probabilities.
%
%



==> Proof_Continuity.tex <==
\subsection{Continuous dependence of solutions on the driver}
%\label{ldpContSec}
%%{\bf for lsc of rate function also needs to be checked for $\nu$ with finite entropy}
%
%In other words, fixing $t\in[0,T]$ we show that for every $\e>0$ there exists an environment $U$ of $\nu$ in the induced topology on $\MM_\mu$ such that if $\nu'\in U$, then $|\b_t(\nu')-\b_t(\nu)|<\e$ holds for all $\nu'\in U$. 
%%In order to prove this claim, we construct an environment $U$ of $\nu$ such that if $\nu'\in U$ then $|\b_t(\nu')-\b_t(\nu)|<\e$.
%This will prove Proposition~\ref{mapContLem}. Let us denote by $$J_{\nu'}=\sup_{t\in[0,T]}\nu'_{\ms{ TU}}(\{t\},[0,1])$$
%the maximal temporal point-mass of $\nu'$ and note that $J_{\nu'}=0$ if $\nu'\in\MM_{\ms{ac}}$. As a first step, we provide bounds for the deviations of the increments 
%$$(\va_{t_2}(\nu)-\va_{t_2}(\nu'))-(\va_{t_1}(\nu)-\va_{t_1}(\nu')),\qquad0\le t_1\le t_2\le T. $$
%
%\begin{lemma}
%	\label{incrLowLem}
%	Let $0\le t_1\le t_2\le T$ and $\nu\in\MM_{\ms{ac}}$ with $r>0$ be arbitrary. Furthermore, let $\nu'\in\MM_\mu$. Then,
%	\begin{align*}
%		&|\va_{t_2}(\nu')-\va_{t_2}(\nu)|-|\va_{t_1}(\nu')-\va_{t_1}(\nu)|\\
%		&\quad\le\nu'_{\ms{TU}}([t_1,t_2]\times[r^{-1}\va_{t_1}(\nu),r^{-1}\va_{t_2}(\nu)])+J_{\nu'}
%		+|\int_{(t_1,t_2]}(\nu'_{\ms{TU}}-\nu_{\ms{TU}})(\d s,(r^{-1}\va_s(\nu),1])|.
%	\end{align*}
%\end{lemma}
%\begin{proof}
%	Write $\va=\va(\nu)$ and $\va'=\va(\nu')$, we observe that
%	\begin{align}
%		\label{tzEq}
%		\begin{split}
%			\va'_{t_2}-\va_{t_2}&=\va'_{t_1}-\va_{t_2}+\int_{(t_1,t_2]}\nu'_{\ms{TU}}(\d s,(r^{-1}\va'_{s-},1])\\
%			&=\va'_{t_1}-\va_{t_1}+\int_{(t_1,t_2]}\nu'_{\ms{TU}}(\d s,(r^{-1}\va'_{s-},1])-\nu_{\ms{TU}}'(\d s,(r^{-1}\va_s,1])\\
%			&\phantom{=}+\int_{(t_1,t_2]}(\nu'_{\ms{TU}}-\nu_{\ms{TU}})(\d s,(r^{-1}\va_s,1]).
%		\end{split}
%	\end{align}
%
%	First, we provide a lower bound for $\va'_{t_2}-\va_{t_2}$. Without loss of generality, we may assume that $\va'_{t_2}<\va_{t_2}$. Then, by monotonicity,
%	\begin{align*}
%		\int_{(t_1,t_2]}\hspace{-0.1cm}\nu_{\ms{TU}}'(\d s,(r^{-1}\va'_{s-},1])-\nu'_{\ms{TU}}(\d s,(r^{-1}\va_{s},1])&\ge\int_{(t_1,t_2]}\hspace{-0.1cm}\nu_{\ms{TU}}'(\d s,(r^{-1}\va_{t_2},1])-\nu_{\ms{TU}}'(\d s,(r^{-1}\va_{s},1])\\
%															      &\ge-\nu'_{\ms{TU}}([t_1,t_2]\times[r^{-1}\va_{t_1},r^{-1}\va_{t_2}]).
%	\end{align*}
%	Second, we provide an upper bound for $\va'_{t_2}-\va_{t_2}$ and may therefore assume $\va'_{t_2}\ge\va_{t_2}$. 
%	Let $t_1^*\in[t_1,t_2]$ denote the infimum of all times $t\ge t_1$ such that $\va'_t\ge\va_{t_1}$. Similarly, we let $t_2^*\in[t_1,t_2]$ denote the supremum of all times $t\le t_2$ such that $\va'_t\le\va_{t_2}$  and set $t_2^*=t_1$ if $\va'_{t_1}>\va_{t_2}$. Then, by monotonicity,
%	\begin{align*}
%		\int_{(t_1,t_2]}\hspace{-0.4cm}\nu_{\ms{TU}}'(\d s,(r^{-1}\va'_{s-},1])-\nu_{\ms{TU}}'(\d s,(r^{-1}\va_s,1])&\le\int_{(t_1,t_2^*]}\hspace{-0.4cm}\nu_{\ms{TU}}'(\d s,(r^{-1}\va'_{s-},1])-\nu_{\ms{TU}}'(\d s,(r^{-1}\va_{s-},1])\\
%		&=\int_{(t_1,t_1^*]}\hspace{-0.4cm}\nu_{\ms{TU}}'(\d s,(r^{-1}\va'_{s-},1])-\nu_{\ms{TU}}'(\d s,(r^{-1}\va_{s-},1])\\
%		&\phantom{=}+\int_{(t_1^*,t_2^*]}\hspace{-0.4cm}\nu_{\ms{TU}}'(\d s,(r^{-1}\va'_{s-},1])-\nu_{\ms{TU}}'(\d s,(r^{-1}\va_{s-},1]).
%	\end{align*}
%	For the first summand, we note that if $t_1^*>t_1$, then
%	\begin{align*}
%		\va'_{t_1}-\va_{t_1}+\int_{(t_1,t_1^*]}\hspace{-0.4cm}\nu_{\ms{TU}}'(\d s,(r^{-1}\va'_{s-},1])=\va'_{t^*_1}-\va_{t_1}\le \nu_{\ms{TU}}'(\{t_1^*\}\times[0,1])\le |\va'_{t_1}-\va_{t_1}|+J_{\nu'}.
%	\end{align*}
%	When leaving out the intermediate step, this inequality certainly remains valid also if $t_1^*=t_1$. Moreover, by the definition of $t_1^*,t_2^*$, we may bound the second summand by
%	\begin{align*}
%		\int_{(t_1^*,t_2^*]}\nu_{\ms{TU}}'(\d s,(r^{-1}\va'_{s-},1])-\nu_{\ms{TU}}'(\d s,(r^{-1}\va_{s-},1])\le\nu_{\ms{TU}}'([t_1,t_2]\times[r^{-1}\va_{t_1},r^{-1}\va_{t_2}]).
%	\end{align*}
%	Inserting these bounds into~\eqref{tzEq} completes the proof.
%\end{proof}
%Using Lemma~\ref{incrLowLem}, we can now provide a proof of Proposition~\ref{mapContLem}.
%\begin{proof}[Proof of Proposition~\ref{mapContLem}]
%	%CHECK.use Lemma incrLowLem
%	%CHECK.use absolute continuity
%%	First, for any $\nu'\in\MM_\mu$, the definition of $\TT_{\nu'}$ implies that
%%	$$\b_T(\nu')\ler'+J_{\nu'}.$$
%%	This yields the claim in the case $r=0$, where we have that $\b(\nu)$ is identically equal to $0$.
%%
%%	We need to show that the map $\nu'\mapsto\b_t(\nu')$ is continuous at $\nu$.  
%Applying Lemma~\ref{incrLowLem} repeatedly to the subdivision $\{0,t/n,\ldots,t\}$ gives that 
%	\begin{align*}
%		&|\va_{t}(\nu')-\va_{t}(\nu)|\le \sum_{i=0}^{n-1}\nu((\tfrac{it}{n},\tfrac{(i+1)t}{n}]\times[r^{-1}\va_{it/n}(\nu),r^{-1}\va_{(i+1)t/n}(\nu)])+nJ_{\nu'}\\
%		&+\sum_{i=0}^{n-1}\Big(|(\nu'-\nu)((\tfrac{it}{n},\tfrac{(i+1)t}{n}]\times[r^{-1}\va_{it/n}(\nu),r^{-1}\va_{(i+1)t/n}(\nu)])|+|\int_{(\tfrac{it}{n},\tfrac{(i+1)t}{n}]}(\nu'-\nu)(\d s,(r^{-1}\va_s(\nu),1])|\Big).
%	\end{align*}
%	By absolute continuity of $\nu$, the first summand is smaller than $\e/3$ if $n$ is sufficiently large. Absolute continuity of $\nu$ also implies that $nJ_{\nu'}<\e/3$  if $\nu'$ is sufficiently close to $\nu$. 	Finally, the continuity of the mapping $\nu'\mapsto\TT_{\nu'}(\b)$ established in Lemma~\ref{tContLem}	shows that the second sum is smaller than $\e/3$ if $\nu'$ is sufficiently close to $\nu$.
%\end{proof}
We start by stating two supporting lemmas which will be proved below. We then first derive the continuity in Lemma~\ref{Cont_Sol}. 
\begin{lemma}\label{NormApproxGen}
For all $\nu\in\MM$, $\de\ge\de'>0$, we have 
$$\Vert\bdde(\nu)-\b^{\de'}(\nu)\Vert\le2\sup_{0\le i\le\lfloor\TF/\de\rfloor}\nu([i\de,(i+1)\de]\times[0,1]).$$
\end{lemma}
\begin{lemma}\label{ContractionDiscrete}
The mappings $\MM\to\LL$ given by $\nu\mapsto\bdde(\nu)$ is continuous w.r.t.~the projective-limit topology and the topology of point-wise convergence at any $\nu\in\MM_{\ms{ac}}$.
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{Cont_Sol}]
Assume $\nu',\nu\in\MM$, $\nu\in\MM_{\ms{ac}}$ and $t\in[0,\TF]$, then for $\de\ge\de'>0$
\begin{equation*}
\begin{split}
|\b_t(\nu)-\b_t(\nu')|\le|\b_t(\nu)-\bdde_t(\nu)|+|\bdde_t(\nu)-\bdde_t(\nu')|+|\bdde_t(\nu')-\b^{\de'}_t(\nu')|+|\b^{\de'}_t(\nu')-\b_t(\nu')|.
\end{split}
\end{equation*}
According to Lemma~\ref{NormApproxGen}, for the second last summand, we can further estimate 
\begin{equation*}
\begin{split}
|\bdde_t(\nu')-\b^{\de'}_t(\nu')|\le 2|(\nu'-\nu)([i\de,(i+1)\de]\times[0,1])|+2\nu([i\de,(i+1)\de]\times[0,1]). 
\end{split}
\end{equation*}
Now, we can pick $\de>0$, sufficiently small, such that $\nu([i\de,(i+1)\de]\times[0,1])\le\e/8$ and $\Vert\b(\nu)-\bdde(\nu)\Vert\le\e/4$. Moreover, by Lemma~\ref{ContractionDiscrete}, there exists an open neighborhood $U$ of $\nu$, such that if $\nu'\in U$ also $ |(\nu'-\nu)([i\de,(i+1)\de]\times[0,1])|\le \e/8$ and $|\bdde_t(\nu)-\bdde_t(\nu')|\le\e/4$. Finally, by the definition of $\b(\nu')$, letting $\de'$ tend to zero, also $|\b^{\de'}_t(\nu')-\b_t(\nu')|$ tends to zero.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{NormApproxGen}]
%	By Lemma~\ref{trivCompLem} it suffices to show that 
%	$$\b_t \le \bdde_t + 3\e$$
%	holds for all $t \in [0, \TF]$.
We proceed by induction on $i$. For $i=0$ $\bdde_0=\bdde_0(\nu)=\b^{\de'}_0(\nu)=\b^{\de'}_0$ and there is nothing show. We assume that for $i_0$,
$$\sup_{t\in[(i_0-1)\de,i_0\de]}|\bdde_t-\b^{\de'}_t|\le2\sup_{0\le i\le\lfloor\TF/\de\rfloor}\nu([i\de,(i+1)\de]\times[0,1])=2\e.$$
Then we conclude for $t\in[i_0\de,(i_0+1)\de]$ as follows. 
Since $\de'\le\de$ we have $\bdde\le\b^{\de'}$. Now, if 
	$\bdde_{i_0\de} + \e\ge \b^{\de'}_{i_0\de}$, then 
	$$\b^{\de'}_t \le \b^{\de'}_{i_0\de} + \nu([i_0\de, t] \times [0,1]) \le (\bdde_{i_0\de} + \e) + \e \le \bdde_{t} + 2\e.$$
	Otherwise, if $\bdde_{i_0\de} + \e\le \b^{\de'}_{i_0\de}$, then 
	$$\bddde_{(i_0+1)\de} = \bdde_{i_0\de} + \nu([i_0\de, (i_0+1)\de] \times [0,1]) \le \b^{\de'}_{i_0\de}.$$
	Hence, 
	\begin{align*}
		\b^{\de'}_t \le \b^{\de'}_{i_0\de} +  \nu([i_0\de, t] \times [\b^{\de'}_{i_0\de}, 1])\le \b^{\de'}_{i_0\de} +  \nu([i_0\de, t] \times [\bddde_{(i_0+1)\de}, 1])
		=  \b^{\de'}_{i_0\de} + \bdde_{t} - \bdde_{i_0\de},
	\end{align*}
	so that the assertion follows from the induction hypothesis.
\end{proof}




\begin{proof}[Proof of Lemma~\ref{ContractionDiscrete}]
%[Proof of Lemma~\ref{ContractionDiscrete}]

\end{proof}


%\begin{proof}[Proof of Lemma~\ref{Cont_Sol}]
%	Let $\e>0$ be arbitrary, by the absolute continuity of $\nu$, there exists $n\ge1$ such that $\nu([in^{-1}\TF, (i+1)n^{-1}\TF]\times[0,1])\le\e$ for every $i$. We first claim that if $\nu'$ is sufficiently close to $\nu$, then,
%	$$|\b_{in^{-1}\TF}(\nu) - \b^\de_{in^{-1}\TF}(\nu')| \le 3\e$$
%	for all $i$ and sufficiently small $\de=\de(\nu')>0$. We will only show that $\b_{in^{-1}\TF}(\nu)-\b_{in^{-1}\TF}(\nu')  \le 3\e$. The other direction is obtained using similar arguments. Let $i\le \TF n$ be arbitrary and let $i_1$ denote the last index before $i$ such that 
%	$$\b_{i_1n^{-1}\TF}(\nu) - \b_{i_1n^{-1}\TF}(\nu') \le \e$$
%	and put $i_2 = i_1 + 1$. Such $0\le i_1<i$ exists since $\b_{0}(\nu) =0= \b_{0}(\nu')$.
%	%if we assume $\nu'$ to be sufficiently close to $\nu$ such that $|(\nu'-\nu)([0, n^{-1}\TF]\times[0,1])|\le\e$. 
%	Then we have,
%	$$\b_{i_2n^{-1}\TF}(\nu) \le \b_{i_1n^{-1}\TF}(\nu) + \nu([i_1n^{-1}, i_2n^{-1}]\times [0,1]) \le (\b_{i_1n^{-1}\TF}(\nu') + \e) + \e\le\b_{i_2n^{-1}\TF}(\nu') +2\e.$$
%	Moreover, we have
%	\begin{align*}
%\b_{in^{-1}\TF}(\nu) - \b_{in^{-1}\TF}(\nu')= &\, \b_{i_2n^{-1}\TF}(\nu) - \b_{i_2n^{-1}\TF}(\nu') \cr
%&+\sum_{j = i_2}^{i - 1}\Big(\big(\b_{(j + 1) n^{-1}\TF}(\nu) - \b_{(j + 1) n^{-1}\TF}(\nu')\big) - \big(\b_{jn^{-1}\TF}(\nu) - \b_{jn^{-1}\TF}(\nu')\big) \Big)
%%&+\sum_{j = i_2}^{i - 1}[\int_{jn^{-1}\TF}^{(j+1)n^{-1}\TF} \nu(\d t, [\b_{t}(\nu), 1])
%%-\int_{jn^{-1}\TF}^{(j+1)n^{-1}\TF} \nu'(\d t, [\b_{t}(\nu'), 1])]
%\end{align*}
%and, by the definition of $i_1$, $\b_{jn^{-1}\TF}(\nu) -\b_{jn^{-1}\TF}(\nu') > \e$ for all $i_2\le j< i$. In particular, 
%\begin{align*}
%\b_{(j+1)n^{-1}\TF}(\nu')+\e<\b_{(j+1)n^{-1}\TF}(\nu)\le\e+\b_{jn^{-1}\TF}(\nu)
%\end{align*}
%and thus $\b_{(j+1)n^{-1}\TF}(\nu')\le\b_{jn^{-1}\TF}(\nu)$, which implies
%\begin{align*}
%\int_{jn^{-1}\TF}^{(j+1)n^{-1}\TF}\nu'(\d t, [\b_{t}(\nu), 1])&\le \nu'([jn^{-1}\TF,(j+1)n^{-1}\TF], [\b_{jn^{-1}\TF}(\nu), 1])\cr
%%&\le \nu'([jn^{-1}\TF,(j+1)n^{-1}\TF], [\b_{jn^{-1}\TF}(\nu'), 1])-\nu'([jn^{-1}\TF,(j+1)n^{-1}\TF], [\b_{jn^{-1}\TF}(\nu'),\b_{jn^{-1}\TF}(\nu')+\e])\cr
%& \le \nu'([jn^{-1}\TF,(j+1)n^{-1}\TF], [\b_{(j+1)n^{-1}\TF}(\nu'), 1])\cr
%%+\nu'([jn^{-1}\TF,(j+1)n^{-1}\TF], [\b_{(j+1)n^{-1}\TF}(\nu)-\e,\b_{jn^{-1}\TF}(\nu)])\cr
%		&\le \int_{jn^{-1}\TF}^{(j+1)n^{-1}\TF}\nu'(\d t, [\b_{t}(\nu'), 1]).
%\end{align*}
%Using this, we can estimate, 
%\begin{align*}
%		\b_{(j+1)n^{-1}\TF}(\nu) & = \b_{jn^{-1}}(\nu) + \int_{jn^{-1}\TF}^{(j+1)n^{-1}\TF} \nu(\d t, [\b_{t}(\nu), 1])\cr
%		&\le  \b_{jn^{-1}\TF}(\nu) + (\b_{(j + 1) n^{-1}}(\nu') - \b_{jn^{-1}\TF}(\nu')) + \int_{jn^{-1}\TF}^{(j+1)n^{-1}\TF} (\nu - \nu')(\d t, [\b_{t}(\nu), 1]),
%\end{align*}
%which implies
%\begin{align*}
%\b_{in^{-1}\TF}(\nu) - \b_{in^{-1}\TF}(\nu')& \le 2\e + \int_{i_2n^{-1}\TF}^{in^{-1}\TF} (\nu - \nu')(\d t, [\b_{t}(\nu), 1])\cr
%&\le 2\e + \sup_{j\le i} \int_{jn^{-1}\TF}^{in^{-1}\TF} (\nu - \nu')(\d t, [\b_{t}(\nu), 1]).
%\end{align*}
%In particular, by the $\tau$-convergence of $\nu'$ and an application of 
%%Finally, the continuity of the mapping $\nu'\mapsto\TT_{\nu'}(\b)$ established in 
%Lemma~\ref{tContLem}	
%%shows that the second sum is smaller than $\e/3$ if $\nu'$ is sufficiently close to $\nu$.
%the proof is completed.
%\end{proof}
%%
%\begin{align*}
%	\bddde_{t}=\bdde_{(n-1)\de}+\nu_{\ms{T}}\big(((n-1)\de,n\de]\times[0,1]\big)
%\end{align*}
%for $t\in((n-1)\de,n\de]$.
%Then,  for $t\in((n-1)\de,n\de]$ we put 
%\begin{align*}
%	\bdde_{t}=\bdde_{(n-1)\de}+\nu_{\ms{TU}}\big(((n-1)\de,t]\times[r^{-1}\bddde_{n\de},1]\big).
%\end{align*}



==> Proofs_Neu.tex <==
\section{Proof of Theorem \ref{LDP_NoSpatial} }

\subsection{Markovian structure of $B_t$}
Recall that in the setting of Theorem~\ref{LDP_NoSpatial} we only consider the total mass of busy relays and there we simply write $B_t$ instead of $B_t(W)$.
%defined via the equation \eqref{DE_Cont} with 
In this subsection we show that the solutions to equation \eqref{DE_Discrete}, modeled using the random variable $U_j$, is equal to the process of busy relays as defined in \eqref{Busy_Process}.
To make this more precise, let $\tilde B_t$ denote the unique solution of \eqref{DE_Discrete} for the initial condition $\tilde B_0=0$.
\begin{proposition}
The processes $\{B_t\}$ and $\{\tilde B_t\}$ have the same distribution. 
\end{proposition}

\begin{proof}
Let us fix a realization of the spatial location of relays $Y$. Further, let us fix the number $N_{\rm{T}}$ of transmitters together with their data transmission times $\tau=(\tau_i)_{i\in N_{\rm{T}}}$. After that, the process $B_t$ only depends on the random selection of a relay for each transmitter which is done with probability $1/|Y|$. For the process $\tilde B_t$ the randomness comes from the uniform distribution of selection variables $U=(U_i)_{i\in N_{\rm{T}}}$. 

For simplicity we assume the data transmission times to be ordered, then both $B^\tau=\{B_{\tau_i}\}$ and $\tilde B^\tau=\{\tilde B_{\tau_i}\}_{i\in N_{\rm{T}}}$ are time-homogeneous Markov chains. For the transition probability of $B_\tau$ we note that if at time $\tau_i-$, $k$ relays are busy, then at time $\tau_i$, $k+1$ are buys with probability $1-k/|Y|$. With probability $k/|Y|$ at time $\tau_i$ the number of busy relays remains $k$.
As for $\tilde B^\tau$ if at time $\tau_i-$, $k$ relays are busy, then an additional relay becomes busy if $U_{\tau_i}\in[k/|Y|,1]$. Hence the transition probabilities coincide.
\end{proof}


\subsection{The extremal fixed points of the squared integral operator}


\subsubsection{Picard iterations of the integral operator}
In this section we prove the existence of the extremal fixed points $\b^\pm$ of the squared integral operator via a Picard iteration argument. Further, we give an example of a driver $\nu$ with $h(\nu|\mu)<\infty$ such that $\b^+(\nu)>\b^-(\nu)$. This will also provide an example where the equation \eqref{DE_Cont} does not admit a solution. 
%The main idea is to interpret solutions to the equation \eqref{DE_Cont} as fixed points of the operator given by the r.h.s.~of \eqref{DE_Cont}. 
%These fixed points are obtained by a Picard iteration where the convergence can be established using the anti-monotonicity of the operator. This will also give the uniqueness. 
More precisely 
%define for a given measure $\nu$ on $[0,T]\times[0,1]\times M$ the operator $\TT_\nu:\, \LL\to\LL$ via
%\begin{align}\label{DE_Cont_Op}
%\TT_\nu(\b)=\int_0^t\nu_{\rm{T}}(\d s,[\nu_{{\rm{R}}}^{-1}\b_{s-},1])
%\end{align}
%where $\nu_{{\rm{R}}}$ and $\nu_{{\rm{T}}}$ are defined as described above. W
we have the following monotonicity property of $\TT_\nu$ defined in \eqref{IntOp}.
\begin{lemma}\label{Monotonicity}
For $\b_t\ge\b'_t$ for all $t\in[0,T]$ we have $\TT_\nu(\b)\le\TT_\nu(\b')$.
\end{lemma}
\begin{proof}
By the monotonicity of the integrals we have 
\begin{align*}
\TT_\nu(\b)=\int_0^t\int_{\b_{s-}/\nu_{{\rm{R}}}}^1\nu_{\rm{T}}(\d s,\d u)\le \int_0^t\int_{\b'_{s-}/\nu_{{\rm{R}}}}^1\nu_{\rm{T}}(\d s,\d u)=\TT_\nu(\b').
\end{align*}
\end{proof}

Define iteratively $\b^{(n+1)}=\TT_\nu(\b^{(n)})$ with $\b^{(0)}\equiv 0$ and note that by Lemma~\ref{Monotonicity} we have 
\begin{align}\label{Contraction}
\b^{(0)}\le \b^{(2)}\le \dots \le \b^{(3)}\le \b^{(1)}.
\end{align}
Consequently the pointwise limits
$$\b^-=\lim_{n\uparrow\infty}\b^{(2n)}$$
and 
$$\b^+=\lim_{n\uparrow\infty}\b^{(2n+1)}$$
are well defined. Now we show that $\b^\pm$ are indeed extremal solutions of the squared integral operator. 
\begin{lemma}\label{Existence}
For $\nu$ absolutely continuous, we have $\b^+=\TT_\nu(\b^-)$ and $\b^-=\TT_\nu(\b^+)$. Moreover, if $\b=\TT^2_\nu(\b)$ then $\b^+\ge\b\ge\b^-$.
\end{lemma}
\begin{proof}
{\bf{INCORRECT }}First note that if $\b^{(2n)}_t$ converges monotonically to $\b_t$ then also $\b^{(2n)}_{t-}$ converges to $\b_{t-}$ monotonically. Indeed we can show two inequalities, first we have for all $t<s$
\begin{align*}
\lim_{n\uparrow\infty}\b^{(2n)}_{s-}\ge \lim_{n\uparrow\infty}\b^{(2n)}_{t}=\b_{t}
\end{align*}
and therefore taking the $t\uparrow s$ limit on both sides we arrive at 
\begin{align*}
\lim_{n\uparrow\infty}\b^{(2n)}_{s-}\ge \b_{s-}.
\end{align*}
On the other hand 
\begin{align*}
\lim_{n\uparrow\infty}\b^{(2n)}_{s-}\le \lim_{n\uparrow\infty}\lim_{t\uparrow s}\b^{(2n)}_{t}\le \lim_{t\uparrow s}\b_{t}=\b_{s-}.
\end{align*}
Therefore,
\begin{align*}
\lim_{n\uparrow\infty}\one_{[\nu_{{\rm{R}}}^{-1}\b^{(2n)}_{s-},1]}=\one_{[\nu_{{\rm{R}}}^{-1}\b_{s-},1]}
\end{align*}
and hence an application of monotone convergence completes the proof.
\end{proof}

Let us now present an example where $\b^+>\b^-$ for some driver $\nu$ with $h(\nu|\mu)<\infty$ where $\mu=U[0,T]\otimes U[0,1]\otimes(\de_{\rm{T}}+\de_{\rm{R}})$.
\begin{example}
Define $\nu$ via its density w.r.t.~$\mu(\cdot\times\cdot\times\{T\})$ given by 
$$f(t,u)=
\begin{cases}
1/t & u\le 2-2e^{-t}\\
1 & \text{else}
\end{cases}
$$
and set $\nu_{\rm{R}}=1$. Then 
\begin{enumerate}
\item $h(\nu|\mu)<\infty$,
\item $\b^+_t=2-2e^{-t}$ and $\b^-_t=2-2e^{-t}-t$,
\item the operator $\TT_\nu$ does not admit a fixed point in $L$.
\end{enumerate}
TTTBBBAAA

\end{example}

\input{LDPDiscrete}


\subsection{Proof of Theorem~\ref{LDP_NoSpatial} by approximation}
A major part in the proof of Theorem~\ref{LDP_NoSpatial} will be to show that in the setting when $\nu=\Lla$, asymptotically as $\la\to\infty$ and $\delta\to0$ the inequalities appearing in Lemma~\ref{trivCompLem} are not too far from being equalities. 
%More precisely, at one side of the comparison, we replace $\Lla$ by $\Llap$, where $\la^+=(1+\e)\la$ and $\la^-=(1-\e)\la$ for some small $\e>0$.
We now provide a precise statement of this weak converse comparison result.
\begin{lemma}\label{DoLs}
	%There exist functions $f:[0,1]\to[0,\infty)$ and $\delta:[0,1]\to[0,1]$ such that $\lim_{\e\to0}f(\e)=0$ and for all $\delta\in(0,\delta(\e))$ we have that 
Let $F$ be increasing then, 
	$$\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\g(\Lla)))\ge\limsup_{\de\to0}\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\gdde(\Lla))).$$
	and
	$$\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\g(\Lla)))\le\liminf_{\de\to0}\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\gude(\Lla))),$$
\end{lemma}
The proof of Lemma~\ref{DoLs} is the main technical step in our proof of Theorem~\ref{LDP_NoSpatial}. We first present here how Theorem~\ref{LDP_NoSpatial} is implied by Lemma~\ref{DoLs} and proceed with the proof of Lemma ~\ref{DoLs} in the remainder of this section. 
\begin{proof}[Proof of Theorem~\ref{LDP_NoSpatial}]
%CHECK.use Lemmas UpRs,DoRs,UpLs,DoLs
	We only provide the proof of the upper bound as the lower bound is similar. First, Lemma~\ref{DoLs} implies that 
	$$\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\g(\Lla)))\le\liminf_{\de\to0}\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\gude(\Lla))).$$
	Hence, by Varadhan's Lemma, see~\cite[Theorem 4.3.6]{dz98}, the LDP for the discretized frustrated user process established in Proposition~\ref{ContractionDiscrete} yields
	$$\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\gude(\Lla)))\le\liminf_{\de\to0}-\inf_{\nu}\big\{h(\nu|\mu)-F(\gude(\nu))\big\}.$$
	In particular, Lemma~\ref{trivCompLem} implies that
	$$-\inf_{\nu}\big\{h(\nu|\mu)-F(\gude(\nu))\big\}\le -\inf_{\nu}\big\{h(\nu|\mu)-F(\g^-(\nu))\big\}$$
as required.
\end{proof}

\subsection{Proof of Lemma~\ref{DoLs} via coupling}
In order to prove Lemma~\ref{DoLs}, we use a coupling argument. More precisely, we enlarge the probability space $(\Omega,\mc{F},\P)$ to support $\Lla$ together with a coupled version $\Llac$ in a way that there is a not too small probability for $\gude(\Llac)$ to stochastically dominate the original frustrated user process $\g(\Lla)$. In contrast to the classic method of exponential approximation~\cite[Definition 4.2.14]{dz98} it will be critical to control that probability conditioned on $X^\la$ except for an event that is arbitrarily exponentially unlikely. A variant of this technique has already been successfully applied in earlier works~\cite{wireless2}. More precisely, the requirements on the coupling are summarized in the following result.

\begin{lemma}
	\label{couplLem}
	For every $\de,\e>0$ there exists a coupling $\Llac(\e)$ of $\Lla$, events $G^{\ms{d}}(\de,\e,\la)$, $G^{\ms{u}}(\de,\e,\la)$ and $H(\de,\e,\la)$, and a function $f:[0,\infty)\to[0,1]$ with $\lim_{\e\to0}f(\e)=0$ satisfying the following properties. 
	\begin{enumerate}
		\item[]{\bf (DOM)} The bounds
			$$\g(\Llac(\e))\ge\gdde(\Lla)\one\{G^{\ms{d}}(\de,\e,\la)\},\quad\text{ and }\quad
		\gude(\Llac(\e))\ge\g(\Lla)\one\{G^{\ms{u}}(\de,\e,\la)\}$$
		hold almost surely	(domination property),
	\item[]{\bf (SUP)} 
		the events $H(\delta,\e,\la)$ are measurable with respect to $X^\la$ and satisfy
		$$\limsup_{\e\to0}\limsup_{\de\to0}\limsup_{\la\to\infty}\la^{-1}\log\P(H(\delta,\e,\la)^c)=-\infty$$
		(super-exponential decay of pathological-event probabilities), and
	\item[]{\bf (SUB)} the bound
		$$\min\{\P(G^{\ms{d}}(\de,\e,\la)|X^\la),\P(G^{\ms{u}}(\de,\e,\la)|X^\la)\}\ge\exp(-f(\e)\la)\one\{H(\de,\e,\la)\}$$
		holds almost surely for every $\de,\e>0$
		(sub-exponential decay of conditional probabilities). 
	\end{enumerate}
\end{lemma}
In order to lighten the notation, we will drop the references to $(\de, \e,\la)$ in the following.
\begin{proof}[Proof of Lemma~\ref{couplLem}]
	The construction of the coupling will be described in Section~\ref{coupConstSec}, whereas the verification of the conditions is outsourced to Lemmas~\ref{domLem},~\ref{supExpLem} and~\ref{subExpLem}, respectively.
\end{proof}
To conclude this section, we note how Lemma~\ref{couplLem} can be used to deduce Lemma~\ref{DoLs}.
\begin{proof}[Proof of Lemma~\ref{DoLs}]
		As initial remark, by property {\bf (SUP)} 
		\begin{align}
			\label{pathProbEq}
			\limsup_{\de\to0}\limsup_{\la\to\infty}\la^{-1}\log\P(H^c)<-K-F_{\ms{max}}
		\end{align}
		holds for all $K\ge0$ and all sufficiently small $\e=\e(K)>0$. 

                To begin with, we prove the lower bound. Here, it suffices to fix $K\ge0$ arbitrary and show that
                $$\max\{-K,\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\g(\Lla)))\}\ge\limsup_{\de\to0}\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\gdde(\Lla))).$$
                First, by condition {\bf (DOM)}, 
                \begin{align*}
                        &\E[\exp(\la F(\g(\Llac)))]
                        \ge\E[\one\{G^{\ms{d}}\}\exp(\la F(\gdde(\Lla)))]
			\ge\E[\P(G^{\ms{d}}|X^\la)\one\{H\}\exp(\la F(\gdde(\Lla)))].
		\end{align*}
		Moreover, condition {\bf (SUB)} gives that 
		\begin{align*}
			\E[\P(G^{\ms{d}}|X^\la)\one\{H\}\exp(\la F(\gdde(\Lla)))]
			\ge\exp(-f(\e)\la)\E\exp(\la F(\gdde(\Lla)))-\exp(\la F_{\ms{max}})\P(H^c).
                \end{align*}
		Hence, using~\eqref{pathProbEq}, we arrive at 
		$$\max\{-K,\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\g(\Lla)))\}\ge\limsup_{\de\to0}\liminf_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\gdde(\Lla)))-f(\e).$$
		Letting $\e$ tend to 0 completes the proof.
		
		The proof of the upper bound is similar, but for the convenience of the reader, we provide some details. The inequality is trivial if the left-hand side is equal to $-\infty$. Hence, we may assume that the left-hand side is finite and we abbreviate its value by $K$. First, the bound~\eqref{pathProbEq} holds for all sufficiently small $\e=\e(K)>0$. Now, as in the lower bound, condition {\bf (DOM)} gives that
                \begin{align*}
                        \E[\exp(\la F(\gude(\Llac)))]
                        \ge\E[\one\{G^{\ms{u}}\}\exp(\la F(\g(\Lla)))]
			\ge\E[\P(G^{\ms{u}}|X^\la)\one\{H\}\exp(\la F(\g(\Lla)))],
		\end{align*}
		and again, by condition {\bf (SUB)},
		\begin{align*}
			\E[\P(G^{\ms{u}}|X^\la)\one\{H\}\exp(\la F(\g(\Lla)))]
			\ge\exp(-f(\e)\la)\E[\exp(\la F(\g(\Lla)))]-\exp(\la F_{\ms{max}})\P(H^c).
                \end{align*}
		Therefore, an application of~\eqref{pathProbEq} yields that
		$$\limsup_{\la\uparrow\infty}\la^{-1}\log\E\exp(\la F(\g(\Lla)))\le\liminf_{\de\to0}\limsup_{\la\uparrow\infty}\la^{-1}\log\E[\exp(\la F(\gude(\Llac)))]+f(\e),$$
		as  required.
\end{proof}


\subsection{Construction of the coupling}
\label{coupConstSec}

%The first step in the proof of Lemma~\ref{couplLem} is to show that there is a good chance that for $\nu=\Lla$ and small $\de$ the inequalities in Lemma~\ref{trivCompLem} are close to being equalities. 
In order to construct the coupling satisfying conditions {\bf (DOM)}, {\bf (SUB)} and {\bf (SUP)}, we will need additional randomness and therefore introduce suitable couplings of $X^{\la}$. These couplings should provide us with the freedom to adjust the marks of some users that are placed in a particularly unfortunate way. 
To make this precise, we extend the state space from 
$$E=[0,T]\times V$$
to 
$$\Sigma=[0,T]\times\{0,1\}\times V^2,$$
where $V=\burv$ and the additional components have the following interpretation. 
The binary set $\{0,1\}$ indicates the type of the point, i.e.~whether for the coupled Poisson point process, the first or the second copy of the marks $V=\burv$ should be used.

More precisely, we define the coupling Poisson point process $X^{*,\la}$ as a Poisson point process on the space $\Sigma$
with intensity measure given by the product measure
$$\la\big(\LL\otimes((1-\e)\delta_0+\e\delta_1)\otimes\big(U[0,1]\otimes(p_{\ms{R}}\delta_{\ms{R}}+p_{\ms{T}}\delta_{\ms{T}})\otimes(p\delta_{\ms{B}}+(1-p)\delta_{\ms{U}})\big)^{\otimes2}\big).$$
Now, we think of $X^{\la}$ as the point process obtained by first taking the 
image of $X^{*,\la}$  under the projection $\Sigma\to E$
that forgets both the component $\{0,1\}$ as well as the second copy of the marks $V$.
%Moreover, we can decompose $X^{*,\la}$ as
%$$X^{*,\la}=X^{*,\la,0}\cup X^{*,\la,1},$$
%where for $i\in\{0,1\}$ the Poisson point process $X^{*,\la,i}$ consists of the points of $X^{*,\la}$ having $i$ as their first coordinate. Using this notation, 
We define the coupled Poisson point process $X^{\ms{c},\la}$ by first taking the image of the coupling Poisson point process $X^{*,\la}$ under the projection
\begin{align*}
	\Sigma&\to E\\
	(t,b,v^{(0)},v^{(1)})&\mapsto (t,v^{(b)}).
\end{align*}
In other words, the first symbol decides whether to use the standard first or the alternative second copy of the marks $V$.

For this coupling to be useful in the derivation of the lower bound, we distinguish two cases. First, if the number of relays is exceptionally small, then we consider the event where all users in the coupled process are transmitters.
%transmitters in $X^{\la}$ come from type $0$, whereas all relays in $X^{\la}$ come from type $1$ and become transmitters in the coupled process. 
Since there are no more relays in the coupled process, everybody becomes frustrated. 
More precisely,we introduce the sets
\begin{align*}
	A^{\sim}&=\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),(u^{(1)},\bs{\sigma^{(1)}}))\in\Sigma:\,\sigma^{(b)}_{\ms{RT}}=\ms{T})\}
%	A^{\sim}_1&=\{(t,b,v^{(0)},(u^{(1)},\bs{\sigma^{(1)}}))\in\Sigma_1:\,\sigma^{(1)}_{\ms{RT}}=\ms{T})\},
\end{align*}
where $\boldsymbol{\sigma}=(\boldsymbol{\sigma^{(0)}},\boldsymbol{\sigma^{(1)}})=(\sigma_{\ms{RT}}^{(0)},\sigma_{\ms{BU}}^{(0)},\sigma_{\ms{RT}}^{(1)},\sigma_{\ms{BU}}^{(1)})$. Then, we define
	$$G^{\sim}=\{X^{*,\la}\subset A^{\sim}\}.$$


In the second case, we consider the event where in the coupling Poisson point process $X^{*,\la}$ the points are (1) of type $0$ whenever there is a transmitter in the original process $X^{\la}$ who is either blocked or whose first $[0,1]$-mark does not lie between the approximations $\bddde_t(\Lla)/\LlaR$ and $\bdde_t(\Lla)/\LlaR$ and (2) of type 1 and blocked in the coupled process $X^{\ms{c},\la}$, otherwise. 
More precisely, we introduce the random diagonal
$$\Delta^{\ms{d}}=\big\{(t,u)\in[0,T]\times[0,1]:\, \bdde_t(\Lla)/\LlaR\le u\le\bddde_t(\Lla)/\LlaR\big\},$$
as well as, writing $\Sigma_i=\{(t,b,v^{(0)},v^{(1)})\in\Sigma:\,b=i\}$, the disjoint sets
\begin{align*}
	A^{\ms{d}}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),v^{(1)})\in\Sigma_0:\,   \sigma_{\ms{RT}}^{(0)}=\ms{R}\big\},\\
	A^{\ms{d}}_{0}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),v^{(1)})\in\Sigma_0:\,   \sigma_{\ms{RT}}^{(0)}=\ms{T},\,  \big((t,u^{(0)})\not\in\Delta^{\ms{d}} 
	\text{ or }\sigma^{(0)}_{\ms{BU}}=\ms{B}\big)\big\},\\
	A^{\ms{d}}_{1}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),(u^{(1)},\bs{\sigma^{(1)}}))\in\Sigma_1: 
	\, (t,u^{(0)})\in\Delta^{\ms{d}},\,\boldsymbol{\sigma} =(\ms{T},\ms{U},\ms{T},\ms{B})\big\},
\end{align*}
and finally, we put
$$G^{\ms{d}}=\{X^{*,\la}\subset A^{\ms{d}}_{}\cup A^{\ms{d}}_{0}\cup A^{\ms{d}}_{1}\}\cup G^{\sim}.$$

As the upper bound requires one additional iteration of the operator $\mc{T}$, the argument is slightly more involved than in the lower bound. Indeed, suppose that $\b_t(\Lla)$, $\buuude_t(\Lla)$ and $\bude_t(\Lla)$ would agree up to a certain point in time $t$. Now, assume that at $t$ a new transmitter arrives whose $[0,1]$-mark is contained in the interval 
$$[\b_{t}(\Lla)/\LlaR,\bde_t(\Lla)/\LlaR],$$ 
where we define the upper approximation
$$\bde_t(\Lla)=\b_{\lfloor t/\de\rfloor\de}(\Lla)+\Lla([\lfloor t/\de\rfloor\de,\lfloor t/\de\rfloor\de+\de]\times[0,1]).$$
 Then both the original process $\b(\Lla)$ and the approximation $\bude(\Lla)$ would classify the new transmitter as non-frustrated. However, this setting is still problematic as the new transmitter is frustrated w.r.t.~$\buuude(\Lla)$ and this erratic behavior can lead to divergence of the coupled processes at later times. Therefore, in the coupled process the $[0,1]$-mark of the transmitter must be changed such that it becomes non-frustrated also with respect to $\buuude$. This does not cause any problems, unless it is very expensive to put $[0,1]$-marks that are larger than $\bde_{}(\Lla)/\LlaR$. These issues will be resolved by constructing the coupling in such a way that once $\b_t(\Lla)$ comes close to $\LlaR$, in the coupled process all points with marks close to $1$ will be forced to become frustrated.

In the following, we write
$$T_\e=\inf\{t\in[0,T]:\,\b_t(\Lla)/\LlaR\ge1-\e'\}$$
for the first time that $\b_t(\Lla)$ exceeds $1-\e'=1-\exp(-\e^{-2})$.  
We partition the big state space $\Sigma$ into $\Sigma=\Sigma^{(a)}\cup\Sigma^{(b)}$ depending on whether the first coordinate is in $[0,T_\e]$ or $(T_\e,T]$. 
Moreover, we define the random diagonal
$$\Delta^{\ms{u}}=\big\{(t,u)\in[0,T]\times[0,1]:\,\b_{t}(\Lla)/\LlaR\le u\le\bde_t(\Lla)/\LlaR\big\},$$
Then, in order to define the analog $G^{\ms{u}}$ of the event $G^{\ms{d}}$, we need to follow a different strategy depending on whether a transmitter arrives before time $T_\e$ or after that. 

More precisely, we put
\begin{align*}
	A^{\ms{u}}_{}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),v^{(1)})\in\Sigma_0:\,  \sigma_{\ms{RT}}^{(0)}=\ms{R}\big\},\\
	A^{\ms{u},\ms{a}}_{0}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),v^{(1)})\in\Sigma^{\ms{a}}_0:\,  \sigma_{\ms{RT}}^{(0)}=\ms{T},\,  \big((t,u^{(0)})\not\in\Delta^{\ms{u}}		\text{ or }\sigma^{(0)}_{\ms{BU}}=\ms{B}\big)\big\},\\
A^{\ms{u},\ms{b}}_{0}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),v^{(1)})\in\Sigma^{\ms{b}}_0:\, \sigma_{\ms{RT}}^{(0)}=\ms{T},\,  \big(u^{(0)}\le 1-\e' 
	\text{ or }\sigma^{(0)}_{\ms{BU}}=\ms{B}\big)\big\},\\
	A^{\ms{u},\ms{a}}_{1}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),(u^{(1)},\bs{\sigma^{(1)}}))\in\Sigma^{\ms{a}}_1: 
	\, (t,u^{(0)})\in\Delta^{\ms{u}},\,\bs{\sigma}=(\ms{T},\ms{U},\ms{T},\ms{U}),\, u^{(1)}\ge\bde_t(\Lla)/\LlaR\big\},\\
	A^{\ms{u},\ms{b}}_{1}&=\big\{(t,b,(u^{(0)},\bs{\sigma^{(0)}}),(u^{(1)},\bs{\sigma^{(1)}}))\in\Sigma^{\ms{b}}_1: 
				    \,  u^{(0)}\ge1-\e',\,\boldsymbol{\sigma}=(\ms{T},\ms{U},\ms{T},\ms{B}) \big\},
\end{align*}
where we put $\Sigma^{\ms{a}}_i=\{(t,b,v^{(0)},v^{(1)})\in\Sigma_i:\,t\le T_\e\}$ and $\Sigma^{\ms{b}}_i=\{(t,b,v^{(0)},v^{(1)})\in\Sigma_i:\,t>T_\e\}$.

The event $G^{\ms{u}}$ is now defined as 
$$G^{\ms{u}}=\big\{X^{*,\la}\subset  A^{\ms{u}}_{}\cup A^{\ms{u},\ms{a}}_{0}\cup A^{\ms{u},\ms{b}}_{0}\cup A^{\ms{u},\ms{a}}_{1}\cup A^{\ms{u},\ms{b}}_{1}\big\}\cup G^{\sim}.$$


%We say that the coupling $X^{*,\la}$ between $X^{\la}$ and $X^{\ms{c},\la}$  is \emph{$\ms{d}$-successful} (\emph{$\ms{u}$-successful}) if the event $G^{\ms{d}}$ ($G^{\ms{u}}$) occurs. First, we show that in the events of a successful coupling, the upper and lower bounds derived in Lemma~\ref{trivCompLem} are precise.

\subsection{Verification of condition {\bf (DOM)}}
\label{domSec}
In the present section, we verify condition {\bf (DOM)}.
\begin{lemma}
\label{domLem}
The coupling construction in Section~\ref{coupConstSec} satisfies the domination condition {\bf (DOM)}.
\end{lemma}
\begin{proof}
	The domination condition {\bf (DOM)} is satisfied if the event $G^{\sim}$ occurs, as the coupled process does not contain any relays. Hence, any transmitter becomes frustrated.

	Next, we verify the lower bound in the event $G^{\ms{d}}\setminus G^{\sim}$. We claim that in this case, we have not only domination, but in fact equality. That is, we claim that 	
	$$\bdde_{t}(\Lla)=\b_{t}(\Llac)\quad\text{and}\quad\gdde_{t}(\Lla)=\g_{t}(\Llac)\text{ for all $t\in[0,T]$}.$$
	Since the processes under consideration exhibit only a finite number of jumps, we can proceed by induction on $t$. The case $t=0$ is trivial.
	Regarding part (1), assume that there is a jump at $t>0$ and that we have already shown $\b_{t-}(\Llac)=\bdde_{t-}(\Lla)$. Since 
	$$\bdde_{t}(\Lla)=\bdde_{t-}(\Lla)+L_{\la,\ms{T}}(\{t\}\times[\bddde_{t-}(\Lla)/\LlaR,1]\times\{\ms{U}\}),$$
	and
	$$\b_{t}(\Llac)=\b_{t-}(\Llac)+L_{\la,\ms{T}}^{\ms{c}}(\{t\}\times[\b_{t-}(\Llac)/\LlacR,1]\times\{\ms{U}\}),$$
	it suffices to show that 
	\begin{align}
		\label{coupDEq}
		L_{\la,\ms{T}}(\{t\}\times[\bddde_{t-}(\Lla)/\LlaR,1]\times\{\ms{U}\})=L_{\la,\ms{T}}^{\ms{c}}(\{t\}\times[\b_{t-}(\Llac)/\LlacR,1]\times\{\ms{U}\}).
	\end{align}
	First, the event $G^{\ms{d}}\setminus G^{\sim}$ implies that $\LlaR=\LlacR$. Now, we distinguish two cases depending on the value of the mark $\{0,1\}$. As the event $G^{\ms{d}}\setminus G^{\sim}$ occurs, a transmitter of type $0$ is blocked or lies outside the diagonal $\Delta^{\ms{d}}$. In both cases, the two sides of~\eqref{coupDEq} agree. On the other hand, if the transmitter is of type $1$, then the occurrence of the event $G^{\ms{d}}\setminus G^{\sim}$,  implies that the user is contained in $\Delta^{\ms{d}}$ and is also blocked in the second component. In particular, both sides of~\eqref{coupDEq} are equal to $0$.	

	Finally, we verify the upper bound in the event $G^{\ms{u}}\setminus G^{\sim}$. Here, we also prove a sharper result by induction on $t$, namely that $$\bude_{t}(\Llac)=\buuude_{t}(\Llac)=\b_{t}(\Lla)\quad\text{for all $t\in[0,T_\e]$},$$
		and $\gude_{t}(\Llac)\ge\g_t(\Lla) $ for all $t\in[T_\e,T]$. We first consider the case where $t\le T_\e$ and assume that we have already shown that $\b_{s}(\Lla)=\buuude_{s}(\Llac)=\bude_{s}(\Llac)$ for all $s<t$. As above, we need to verify that 
	\begin{align}
		\label{coupUEq1}
		L_{\la,\ms{T}}(\{t\}\times[\b_{t-}(\Lla)/\LlaR,1]\times\{\ms{U}\})=L_{\la,\ms{T}}^{\ms{c}}(\{t\}\times[\buude_{t-}(\Llac)/\LlacR,1]\times\{\ms{U}\})
	\end{align}
	and
	\begin{align}
		\label{coupUEq2}
		L_{\la,\ms{T}}(\{t\}\times[\b_{t-}(\Lla)/\LlaR,1]\times\{\ms{U}\})=L_{\la,\ms{T}}^{\ms{c}}(\{t\}\times[\buuude_{t-}(\Llac)/\LlacR,1]\times\{\ms{U}\}).
	\end{align}
	Again, we conclude from the occurrence of the event $G^{\ms{u}}\setminus G^{\sim}$ that $\LlaR=\LlacR$. Since we know additionally that $\bude_{s}(\Llac)=\b_{s}(\Lla)$ for all $s<t$, we conclude that $\buude_{t-}(\Llac)=\bde_{t-}(\Lla)$. Now, as above, we distinguish two cases depending on the value of the $\{0,1\}$-mark. If the transmitter is of type 0, as the event $G^{\ms{u}}\setminus G^{\sim}$ occurs, the user is blocked or lies outside of the diagonal $\Delta^{\ms{u}}$. In both cases, the two sides of the equations~\eqref{coupUEq1} and~\eqref{coupUEq2} agree. On the other hand, if the transmitter is of type $1$, then occurrence of the event $G^{\ms{u}}\setminus G^{\sim}$ implies that in the first copy of the marks, the transmitter is unblocked in both copys. Moreover, in the first copy it is contained in $\Delta^{\ms{u}}$, whereas in the second copy it is $[0,1]$-mark is larger than $\bde_{t-}(\Lla)/\LlaR=\buude_{t-}(\Llac)/\LlacR$. In particular, both sides of the equations~\eqref{coupUEq1} and~\eqref{coupUEq2} are equal to $1/\la$.

	Finally, we will show by induction that for $t\ge T_\e$
	\begin{align*}
		\gude_{t}(\Llac)&=\gude_{T_\e}(\Llac)+L_{\la,\ms{T}}([T_\e,t]\times [0,1]\times\{\ms{B},\ms{U}\}).
	\end{align*}
This will conclude the proof since for $t\ge T_\e$ we obtain that 
	\begin{align*}
		&\gude_{T_\e}(\Llac)+L_{\la,\ms{T}}([T_\e,t]\times [0,1]\times\{\ms{B},\ms{U}\})
\\						     &\ge\g_{T_\e}(\Lla)+L_{\la,\ms{T}}([T_\e,t]\times[0,1]\times\{\ms{B},\ms{U}\})-\int_{(T_\e,t]}L_{\la,\ms{T}}(\d s,[\b_{s-}(\Lla)/\LlaR,1]\times\{\ms{U}\})\\
		&=\g_t(\Lla),
	\end{align*}
	as required. The induction step consists of verifying that if at time $t\ge T_\e$ a new user appears, and the claim is already shown for all $s\in[T_\e,t)$, then 
	\begin{align}
		\label{lateIndEq}
		L_{\la,\ms{T}}^{\ms{c}}(\{t\}\times[0,1]\times\{\ms{B},\ms{U}\})-L^{\ms{c}}_{\la,\ms{T}}(\{t\}\times[\buuude_{t-}(\Llac)/\LlacR,1]\times\{\ms{U}\})=L_{\la,\ms{T}}(\{t\}\times [0,1]\times\{\ms{B},\ms{U}\}).
	\end{align}
	Under the event $G^{\ms{u}}\setminus G^{\sim}$ we can now argue as follows. If the considered user is a receiver, then it must be of type $0$ and therefore both sides of~\eqref{lateIndEq} are equal to $0$. Otherwise, the right-hand side and the first expression on the left-hand side of~\eqref{lateIndEq} are equal to $1/\la$, so that it remains to show that
	$$L^{\ms{c}}_{\la,\ms{T}}(\{t\}\times[\buuude_{t-}(\Llac)/\LlacR,1]\times\{\ms{U}\})=0.$$
	This is true if the arriving transmitter is of type $1$ as the event $G^{\ms{u}}\setminus G^{\sim}$ occurs. Finally, under $G^{\ms{u}}\setminus G^{\sim}$ if the transmitter is of type $0$, then it is blocked or
	$$u^{(0)}< 1-\e'\le \b_{T_\e}(\Lla)/\LlaR=\buuude_{T_\e}(\Llac)/\LlacR\le\buuude_{t-}(\Llac)/\LlacR,$$
	as required.
\end{proof}

\subsection{Verification of condition {\bf (SUP)}}
	\label{diagBoundSec}
	In the present section, we introduce the the events $H$ and show that condition {\bf (SUP)} is satisfied. 
%	$$L^{\la}_{\ms{max},\delta}=\max_{0\le i\le T/\de-1}\bde_{i\de}(\Lla)-\b_{i\de}(\Lla)$$
%	denote maximum number of transmitters arriving in one of the intervals $[i\de,(i+1)\de]\times[0,1]$. 
	Then, the event $H(\de,\e)$ will encode that $X^{\la}$ does not contain too many points in certain sets. More precisely, we put 
	\begin{align}
		\label{hDefEq}
		H=H_{\ms{tot}}\cap H_{\ms{top}}\cap H_{\ms{max}}\cap H_{\ms{d}}\cap H_{\ms{u}},
	\end{align}
	where for $\e'=\exp(-\e^{-2})$,
	\begin{align*}
		H_{\ms{tot}}&=\{\Lla(W)\le\e^{-1/2}\},\\
		H_{\ms{top}}&=\{\Lla([0,T]\times[1-\e',1])\le\e\},\\
		H_{\ms{max}}&=\{\max_{0\le i\le T/\de}\Lla([i\de,(i+1)\de]\times[0,1])\le(\e')^2\},\\
		H_{\ms{d}}&=\{\Lla(\Delta^{\ms{d}})\le\e'\}\cup\{\LlaR\le\e\},\\
		H_{\ms{u}}&=\{\Lla(\Delta^{\ms{u}})\le\e'\}\cup\{\LlaR\le\e\}.
	\end{align*}
	As the main result of this section, we show that the complements of the events become arbitrarily exponentially unlikely.
	\begin{lemma}
		\label{supExpLem}
		Using the definition of $H$ given in~\eqref{hDefEq}, condition {\bf (SUP)}  is satisfied.
	\end{lemma}
	\begin{proof}
		We deal with the events $H_i$ one by one. We use the Poisson-concentration inequality~\cite[Chapter 2.2]{lugosi}. The first claim is deduced from the inequality
		$$\P(H_{\ms{tot}}^c)\le\exp\Big(-\la\big(\e^{-1/2}\log(\e^{-1/2}/\mu([0,T]))-\e^{-1/2}+\mu([0,T])\big)\Big).$$
		For the second claim, 
		\begin{align*}
			\P(H_{\ms{top}}^c)&\le\exp\Big(-\la\big(\e \log(\e/(\e'\mu([0,T])))-\e+\e'\mu([0,T])\big)\Big) \\
			&\le\exp(-\e^{-1}\la)\exp\Big(-\la\big(\e\log(\e/\mu([0,T]))-\e+\e'\mu([0,T])\big)\Big).
		\end{align*}
		Moreover, we note that for sufficiently small $\delta$,
		\begin{align*}
			\P(H^c_{\ms{max}})\le\sum_{i=0}^{T/\de-1}\exp\Big(-\la\big((\e')^2\log((\e')^2/\mu([i\de,(i+1)\de]))-(\e')^2+\mu([i\de,(i+1)\de])\big)\Big),
		\end{align*}
		which yields the third claim.

		As a last step, we prove the fourth assertion, as the arguments for the fifth are similar. First,		we claim that 
		\begin{align}
			\label{diagBoundEq}
			\P(H_{\ms{d}}^c)\le \P\big(\big\{\sum\nolimits_{i=0}^{T/\de-1}U_i>\e'\la\big\}\cap\big\{\LlaR>\e\big\}\big),
		\end{align}
		where the $\{U_{i}\}$ are random variables that are independent when conditioned on the $\sigma$-algebra $\mc{F}$ generated by $\LlaR$ and $\{Z_k\}_{0\le k\le T/\de-1}$ and where we put $Z_i=\#(X_{\ms{T}}\cap ([i\de,(i+1)\de]\times[0,1]))$. Moreover, conditioned on $\#X^{\la}_{\ms{R}}$ and $\{Z_k\}_{0\le k\le T/\de-1}$, the distribution of $U_i$ is binomial with $Z_i$ trials and success probability $p_i=\min\{1,Z_i/\#X^{\la}_{\ms{R}}\}$.
		In order to establish~\eqref{diagBoundEq}, we provide an inductive proof of the more general claim
		$$\P(H^c_{\ms{d}})\le\P\big(\big\{N_k+\sum\nolimits_{i=k+1}^{T/\de-1}U_{i}>\e'\la\big\}\cap\big\{\LlaR>\e\big\}\big),$$
		where 
		$$N_k=\#(X^{\la}_{\ms{T}}\cap\Delta^{\ms{d}}\cap[0,k\de])$$
		denotes the number of diagonal transmitters up to time $k\de$. The statement is trivial if $k=T/\de$. Now, in order to perform the backward induction it suffices to show that conditioned on the $\sigma$-algebra $\mc{F}_k$ generated by $X^{\la}\cap([0,k\de]\times[0,1])$ and $\mc{F}$, the $k$th increment $N_{k+1}-N_{k}$ of the diagonal users is stochastically dominated by a binomial distribution of $Z_k$ trials and success probability $p_i$. By the definition of the diagonal $\Delta^{\ms{d}}$, we note that $N_{k+1}-N_k$ is bounded above by 
		$$\#(X^{\la}_{\ms{T}}\cap([k\de,(k+1)\de]\times[\bdde_{k\de}(L_\la)/\LlaR,\bdde_{k\de}(L_\la)/\LlaR+\min\{1,Z_k/\#X^{\la}_{\ms{R}}\}])).$$
		By the Poisson assumption, conditioned on $\mc{F}_k$ this random variable follows a binomial distribution with $Z_k$ trials and success probability at most $p_k$, as required. 

		Therefore, it remains to show that 
		$$\limsup_{\de\to0}\limsup_{\la\to\infty}\frac{1}{\la}\log\P\big(\big\{\sum\nolimits_{i=0}^{T/\de-1}U_{i}>\e'\la\big\}\cap\big\{\LlaR>\e\big\}\big)=-\infty.$$
		We prove this claim by fixing an arbitrary $K_0>0$ and showing that the l.h.s.~is smaller than $-K_0$. First, we distinguish between the cases $Z_i\le K_1\de \la$ and $Z_i\ge K_1\de\la$, where $K_1=K_1(K_0,\e)$ will be chosen below. First, we note that conditioned on $\mc{F}$, the sum $\sum_{i=0}^{T/\de-1}U_i\one\{Z_i\le K_1\de\la\}$ is stochastically dominated by a binomial random variable with $TK_1\la$ trials and success probability $\min\{1,K_1\de/\LlaR\}$. In particular,
		$$\P\Big(\big\{\sum\nolimits_{i=0}^{T/\de-1}U_i\one\{Z_i\le K_1\de\la\}>\e'\la/2\big\}\cap\big\{\LlaR>\e\big\}\Big)\le\P(\ms{Bin}(TK_1\la,K_1\de/\e)>\e'\la/2).$$
		Now, the binomial concentration inequality shows that 
		$$\limsup_{\la\to\infty}\frac{1}{\la}\log\P(\ms{Bin}(TK_1\la,2K_1\de/\e)>\e'\la/2)\le -K_0,$$
		provided that $\de>0$ is sufficiently small.

		Hence, it remains to estimate the probability
		$$\P\Big(\sum\nolimits_{i=1}^{T/\de}Z_i\one\{Z_i> K_1\de\la\}>\e'\la/2\Big).$$

		Now, using exponential Markov and the independence of the Poisson point process, this probability is bounded above by
		\begin{align}
			\label{diagBoundEq2}
		\exp(-K_0\la/2)\prod_{i=1}^{T/\delta}\E\exp(Z_i\one\{Z_i>K_{1}\de\la\}K_0/\e').
	\end{align}
		First, by Varadhan's lemma~\cite[Lemma 10.3.6]{dz98}, 
		\begin{align*}
			&\limsup_{\la\to\infty}\tfrac1\la\log\E\exp(Z_i\one\{Z_i\ge K_{1}\de\la\}K_0/\e')\\
			&\quad\le\sup_{z\ge0}\Big\{z\one\{z\ge K_{1}\de\big\}K_0/\e-z\log(z/\mu([i\de,(i+1)\de]))+z-\mu([i\de,(i+1)\de])\Big\}\\
			&\quad=\max\Big\{0,\sup_{z\ge K_{1}\de}\Big\{-z\log(ze^{-1-K_0/\e}/\mu([i\de,(i+1)\de]))-\mu([i\de,(i+1)\de])\Big\}\Big\}.
	\end{align*}
	If $K_1\ge e^{1+K_0/\e'}\de^{-1}\mu([i\de,(i+1)\de])$, then the inside supremum is negative, so that 
	\begin{align*}
			\limsup_{\la\to\infty}\tfrac1\la\log\E\exp(Z_i\one\{Z_i\ge K_{1}\de\la\}K_0/\e')=0.
	\end{align*}
	Inserting this estimate into~\eqref{diagBoundEq2} completes the proof.
	\end{proof}



\subsection{Verification of condition {\bf (SUB)}}
Finally, in the present section, we show that condition {\bf (SUB)} is satisfied.
\begin{lemma}
	\label{subExpLem}
	There exists a function $f:[0,\infty)\to[0,1]$ with $f(\e)\to0$ for $\e\to0$, such that condition {\bf (SUB)} is satisfied.
\end{lemma}
\begin{proof}
	Conditioned on $X^{\la}$, the probability that every transmitter is of type $0$ in the coupling process $X^{*,\la}$ and that every relay in $X^{\la}$ is a transmitter in the coupled process $X^{\ms{c},\la}$ is given by 
	$$(1-\e)^{\#X^{\la}_{\ms{T}}}(\e p_{\ms{T}})^{\#X^{\la}_{\ms{R}}}.$$
	Hence, if $\{\LlaR\le\e\}$ and the event $H_{\ms{tot}}$ occurs, then 
	$$\P(G^{\sim}|X^{\la})\ge\exp\big(\la(\e^{-1/2}\log(1-\e)+\e\log(\e p_{\ms{T}}))\big).$$
	Hence, in the following, it suffices to work under the event $\{\LlaR>\e\}$.

		As an initial remark, note that, conditioned on $X^\la$, the probability that every relay in $X^{\la}$ is of type 0  in the coupling process $X^{*,\la}$ is given by 
		$$(1-\e)^{\#X^{\la}_{\ms{R}}}.$$
		Regarding $\P(G^{\ms{d}}|X^{\la})$, conditioned on $X^{\la}$, the probability that every transmitter in $X^{\la}$ that is blocked or located outside $\Delta^{\ms{d}}$ is of type $0$ is at least 
		$$(1-\e)^{\#X^{\la}_{\ms{T}}}.$$
		Similarly, the probability that every unblocked transmitter in $\Delta^{\ms{d}}$ is of type $1$ and is contained in $A^{\ms{d}}_{1}$ is bounded below by
		$$(\e p_{\ms{B}}p_{\ms{T}})^{\#(X^{\la}_{\ms{T}}\cap\Delta^{\ms{d}})}.$$
		Hence, under the event $H_{\ms{tot}}\cap H_{\ms{d}}$, 
		 $$\frac{1}{\la}\log\P(G^{\ms{d}}|X^{\la})\ge\e^{-1/2}\log(1-\e)+\e'\log(\e p_{\ms{B}}p_{\ms{T}}).$$

		 Regarding $\P(G^{\ms{u}}|X^{\la})$, we have to consider the times before and after $T_\e$ separately. First, we start with the times before $T_\e$. Conditioned on $X^{\la}$, the probability that every transmitter appearing before time $T_\e$ that is blocked or outside $\Delta^{\ms{u}}$ is of type $0$ is at least
		$$(1-\e)^{\#X^{\la}_{\ms{T}}}.$$
		Similarly, conditioned on $X^{\la}$, the probability that every unblocked transmitter in $\Delta^{\ms{u}}$ which appears before time $T_\e$ is of type $1$ and contained in $A^{\ms{u,a}}_{1}$, is at least
		$$\Big(\e\big(\e'-\max_{0\le i\le T/\de}\Lla([i\de,(i+1)\de]\times[0,1])/\LlaR\big)_+\, p_{\ms{U}}p_{\ms{T}}\Big)^{\#(X^{\la}_{\ms{T}}\cap\Delta^{\ms{u}})}.$$
		Indeed, if $n\de\le T_\e$, then 
		\begin{align*}
			1-\bde_{n\de}/\LlaR&=1-\b_{n\de}/\LlaR-(\bde_{n\de}-\b_{n\de})/\LlaR			\ge\e'-\Lla([n\de,(n+1)\de]\times[0,1])/\LlaR.
		\end{align*}

		For transmitters arriving after time $T_\e$, conditioned on $X^{\la}$, the probability that every transmitter that is blocked or has $[0,1]$-mark below $1-\e'$ is of type $0$ is bounded below by
		$$(1-\e)^{\#X^{\la}_{\ms{T}}}.$$
		Finally, the probability that every unblocked transmitter appearing after time $T_\e$ that has $[0,1]$-mark greater than $1-\e'$ is of type 1 and contained in $A^{\ms{u,b}}_{1}$ is at least
		$$(\e p_{\ms{B}}p_{\ms{T}})^{\#(X^{\la}_{\ms{T}}\cap([0,T]\times[1-\e',1]))}.$$
		In particular, under the event $H$ we have that 
	\begin{align*}
		\frac{1}{\la}\log\P(G^{\ms{u}}|X^{\la})\ge2\e^{-1/2}	\log(1-\e)	+\e'\log(\e p_{\ms{U}}p_{\ms{T}}\e'/2)      +\e\log(\e p_{\ms{B}}p_{\ms{T}}),
	\end{align*}
	as required.
	\end{proof}






==> PropositionMultidomain.tex <==


\begin{proof}[Proof of Proposition~\ref{LDP_Spatial_1}]


	We start with the lower bound. Fix an arbitrary ${\bf r}\ge0$ and assume that ${\bf r_{\la}}$ converges to ${\bf r}$ from below
	Then, 
	\begin{align*}
		\E[\exp(F(\lambda\Gamma^\lambda))]\ge \P[{\bf R_{\la}=r_{{\la}}}]\E[\exp(F(\lambda\gamma(X^\la_{\ms{TR}}(l_{\bf y,r_{\la}}),l_{{\bf r_{{\la}}}})))]
		\ge \P[{\bf R_{\la}=r_{{\la}}}]\E[\exp(F(\lambda\gamma(X^\la_{\ms{TR}}(l_{\bf y,r_{\la}}),l_{{\bf r}})))]\\
		\ge \P[{\bf R_{\la}=r_{{\la}}}]\E[\one\{X^\la_{\ms{TR}}(l_{\bf y,r})=X^\la_{\ms{TR}}(l_{\bf y,r_{\la}})\}\exp(F(\lambda\gamma(X^\la_{\ms{TR}}(l_{\bf y,r}),l_{{\bf r}})))]
	\end{align*}
	Now, we condition on $X^\la_{\ms{TR}}(l_{\bf y,r})$ to obtain that
	$$\E[\one\{X^\la_{\ms{TR}}(l_{\bf y,r})=X^\la_{\ms{TR}}(l_{\bf y,r_{\la}})\}\exp(F(\lambda\gamma(X^\la_{\ms{TR}}(l_{\bf y,r}),l_{{\bf r}})))]$$
	is at least 
	\begin{align*}
		\exp(-\la|r-r_\la|)\E\exp(F(\lambda\gamma(X^\la_{\ms{TR}}(l_{\bf y,r}),l_{{\bf r}}))),
	\end{align*}
	as required.

	Now, to the upper bound. Here, we have to discretize and then consider the cases, where $R_{\la,n}$ is contained in an interval with left coordinate given by $\la^{-1}\lfloor \la i\delta\rfloor$. 
	In particular,
	$$\E[\one\{{\bf R_{\la}}\in[a(i,\la,\delta),]\}\exp()]\le\E[\one\{{\bf R_{\la}}\in[a(i,\la,\delta),]\}\exp(F\gamma(X({\bf R_\la}),l_{a(i,\la,\delta)})]$$

	Now, we note that 
	
	\begin{align*}
	\E[\one\{{\bf R_{\la}}\in[a(i,\la,\delta),]\}\exp(F\gamma(X(l_{a(i,\la,\delta)}),l_{a(i,\la,\delta)})]\\
	=\E[\one\{{\bf R_{\la}}\in[a(i,\la,\delta),]\}\one\{X(R_\la)=X\}\exp(F\gamma(X({\bf R_\la}),l_{a(i,\la,\delta)})]
\end{align*}
Now, we condition the last line on ${\bf R_\la}$  and $X({\bf R_\la})$. Thus, we obtain the lower bound
$$\exp(-\la\delta)\E[\one\{{\bf R_{\la}}\in[a(i,\la,\delta),]\}\exp(F\gamma(X({\bf R_\la}),l_{a(i,\la,\delta)})]$$,
as required.



	The idea of proof is to evaluate the expectation on the left-hand side in two steps. First, we condition on the relays $X_{\ms{R}}$ and use Lemma~\ref{renormLem} together with Theorem~\ref{LDP_NoSpatial} to control the conditional expectation. Second, we use a Varadhan-type argument to determine the limiting behavior when averaging over $X_{\ms{R}}$. To simplify notation, we write $R_{\la,n}=\#(X_{\ms{R}}\cap W_n)$, $1\le n\le l$ and ${\bf R_{\la}}=\{R_{\la,n}\}_{1\le n\le k}$

	First, conditioned on the event $\{{\bf R_{\la}}={\bf r_{\la}}\}$ the transmitters choosing a relay in $W_n$ form a Poisson point satisfying the conditions of Theorem~\ref{LDP_NoSpatial}. Moreover, for different values of $n$ these Poisson point processes are independent. Hence, 

	For the first step, we note that Proposition~\ref{LDP_NoSpatial} implies that 
	$$\limsup_{\la\to\infty}\E[\exp(F(\lambda\Gamma^\lambda))|{\bf R_{\la}=r_{{\la}}}]\le-\inf_{{\bs \nu}\in\MM_{\ms{lc}}}\{h({\bs \nu}|{\bs \a_{r}})-F(\g({\bs \nu},{\bs r}))\} $$
	and 
	$$\liminf_{\la\to\infty}\E[\exp(F(\lambda\Gamma^\lambda))|{\bf R_{\la}=r_{{\la}}}]\ge-\inf_{{\bs \nu}\in\MM_{\ms{lc}}}\{h({\bs \nu}|{\bs \a_{r}})-F(\g({\bs \nu},{\bs r}))\},$$
	where $r_{i,\la}=\la^{-1}\lfloor \la r_i\rfloor$.

	Note that on the left-hand side we condition on $k$ independent Poisson random variables. In order to prove Proposition~\ref{LDP_Spatial_1} we proceed inductively and remove the conditions stepwise. 
	More precisely, writing ${\bf R_{\la,n}}=\{R_{\la,i}\}_{n\le i\le k}$ we claim that for every $n\in\{2,\ldots,k+1\}$,

	\begin{align*}
		&\limsup_{\la\to\infty}\tfrac1\lambda\log\E[\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}]\\
		&\quad\le\sup_{r\ge0}\Big\{-h(r|\mu_{\ms{R}}(W_{n-1}))+\limsup_{\la\to\infty}\tfrac1\lambda\log\E[\exp(F(\lambda\Gamma^\lambda))|R_{\la,{n-1}}=\frac{\lfloor r\la\rfloor}{\la},{\bf R}_{\la,n}={\bf r}_{\la,n}]\Big\},
\end{align*}
	and
	\begin{align*}
		&\liminf_{\la\to\infty}\tfrac1\lambda\log\E[\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}]\\
		&\quad\ge\sup_{r\ge0}\Big\{-h(r|\mu_{\ms{R}}(W_{n-1}))+\liminf_{\la\to\infty}\tfrac1\lambda\log\E[\exp(F(\lambda\Gamma^\lambda))|R_{\la,{n-1}}=\frac{\lfloor r\la\rfloor}{\la},{\bf R}_{\la,n}={\bf r}_{\la,n}]\Big\},
\end{align*}
	
For the upper bound, let $\delta>0$ be arbitrary. Then, by monotonicity,
	\begin{align*}
		&\limsup_{\la\to\infty}\tfrac1\la\log\E[\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}]\\
		&\quad=\limsup_{\la\to\infty}\tfrac1\la\log\E[\one\{R_{\la,n-1}\le\mu_{\ms{R}}(W_{n-1})\}\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}].
	\end{align*}
	Moreover, again by monotonicity,
	\begin{align*}
		&\E[\one\{R_{\la,n-1}\le\mu_{\ms{R}}(W_{n-1}\de)\}\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}]\\
		&\quad=\sum_{i=0}^{\de^{-1}\mu_{\ms{R}}(W_{n-1})} \E[\one\{R_{\la,n-1}\in[a(i,\la,\de),a(i+1,\la,\de))\}\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}],
	\end{align*}
	where $a(i,\la,\de)=\lfloor i\la\de\rfloor\la^{-1}$. Now, we let $R'_{\la,n-1}=a(i,\la,\de)$ where $i$ is determined such that $R_{\la,n-1}\in[a(i,\la,\de),a(i+1,\la,\de))$ and put $R''_{\la,n-1}=R_{\la,n-1}-R'_{\la,n-1}$. Then, ,
	\begin{align*}
		&\quad\le\sum_{i=0}^{\de^{-1}\mu_{\ms{R}}(W_{n-1})} \P(R_{\la,n-1}\in[i\de,(i+1)\de))\E\big[\exp(F(\lambda\Gamma^\lambda))|R_{\la,n-1}=\frac{\lfloor {i\de^{-1}\la}\rfloor}{\la},{\bf R}_{\la,n}={\bf r}_{\la,n}\big].
	\end{align*}
	Now, the large-deviation principle for Poisson random variables~\cite[Lemma 1.2]{penrose} implies that
	$$\limsup_{\la\to\infty}\tfrac1\la\log\P(R_{\la,n-1}\in[i\de,(i+1)\de))=-h((i+1)\de|\mu_{R}(W_{n-1})).$$
	Therefore, the proof of the upper bound is complete once we show that 
	$$\sup_{0\le i\le  \de^{-1}\mu_{\ms{R}}(W_{n-1})}|h((i+1)\de|\mu_{R}(W_{n-1}))-h(i\de|\mu_{R}(W_{n-1}))|.$$
	Now, a quick computation shows that the expression inside the supremum is bounded above by
	$$ \de(1+\mu_{\ms{R}}(W_{n-1})-\log\mu_{\ms{R}}(W_{n-1})),$$
	as required.

	The arguments for the lower bound are similar. Nevertheless, we provide some details for the convenience of the reader and fix an arbitrary $r\ge0$. Then,
	\begin{align*}
		\E[\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}]
		&\ge\E[\one\{R_{\la,n-1}=\la^{-1}\lfloor r\la\rfloor \}\exp(F(\lambda\Gamma^\lambda))|{\bf R}_{\la,n}={\bf r}_{\la,n}]\\
		&=\P(R_{\la,n-1}=\la^{-1}\lfloor r\la\rfloor)\E\big[\exp(F(\lambda\Gamma^\lambda))|R_{\la,n-1}=\la^{-1}\lfloor r\la\rfloor,{\bf R}_{\la,n}={\bf r}_{\la,n}\big].
	\end{align*}
	Hence, the asserted lower bound is a consequence of large-deviation theory for Poisson random variables.
\end{proof}


==> ldp.tex <==
In order to prove Theorem~\ref{mainLDPThm}, we use the contraction principle. First, the random input for the model consists of an iid family $\{(\tau_i,U_i)\}_{1\le i\le\vNa}$ of data arrival times $\tau_i$ together with the decision variables $U_i$. The \emph{empirical measure} $L_N=\vNa^{-1}\sum_{1\le i\le\vNa}\delta_{(\tau_i,U_i)}$ a sufficient amount of randomness in the network, in the sense that given this information, it is possible to construct the dynamics of the proportion of frustrated users by a deterministic rule. By Sanov's theorem~\cite[]{dz98} the empirical measure $L_N$ satisfies a large deviation principle in the $\tau$-topology. In particular, the contraction principle~\cite[]{dz98} allows us to reduce the proof of Theorem~\ref{mainLDPThm} to the statement that the dynamics of frustrated users depends continuously on the input data $L_N$.

Since it is easier to derive the evolution of the busy relays than the one of the frustrated users, we concentrate on the former. By the definition of the dynamic network, the evolution of busy relays can be recovered deterministically from $L_N$. In order to apply the contraction principle, as a first step, in Section~\ref{ldpDefSec}, we show that the dynamics of the proportion of frustrated users can be exressed as $\Phi(L_N)$, where $\Phi:\,\mc{M}_1([0,T]\times W)\to\mc{M}(\mc{D}([0,1]])$ extends the construction rule from empirical measures to arbitrary Borel probability measures on $\mc{M}_1([0,T])$. In a second step, in Section~\ref{ldpContSec}, we show that $\Phi$ is weakly continuous.

\subsection{Definition}
\label{ldpDefSec}
%CHECK.define operator T
%CHECK.show existence and uniqueness
%CHECK.behavior for empirical measure as input
In order to describe the evolution of busy users $\{\va_t\}_{0\le t\le T}$, we observe that the increase of busy users at a given time $t$ depends on the proportion of busy relays at that time. Indeed, initially all relays are idle, so that every incoming user turns an idle relay into a busy one. As time proceeds, the proportion of busy relays grows and it becomes increasingly likely that an incoming user chooses a relay that is busy already. In that case, the user becomes frustrated and does not contribute to the growth of busy relays. 

This description suggests that the evolution of busy users is described by a differential equation driven by the measure $\Lambda(\d t,\d u)$ of incoming users. More precisely,
\begin{align}
	\label{diffEq}
	\va_t=\int_{[0,t]}\Lambda(\d s,[0,1-a_{s-}])
\end{align}

The function $\Phi$ should map the measure of incoming users to the solution of~\eqref{diffEq}. Therefore, we need to guarantee existence and uniqueness of the solutions of~\eqref{diffEq} for arbitrary $\Lambda\in $.

As an auxiliary result, we note that in the case where $\Lambda$ has a density, the solution $\{\va_t\}_{0\le t\le T}$ is continuous in $t$.
\begin{lemma}
	\label{solContLem}
	Let $\lambda(\cdot,\cdot)$ be as in Lemma~\ref{mapContLem}. Then, the solution $\{\va_t\}_{0\le t\le T}$ is continuous in $t$.
\end{lemma}
\begin{proof}
	TBA.
\end{proof}


\subsection{Continuity}
\label{ldpContSec}
In order to prove the continuity of $\Phi$, we need to show that the solutions of~\eqref{diffEq} depend continuously on the input measure $\Lambda$. In fact, by~\cite[]{dz98} it suffices to check continuity for measures of the $\Lambda$ that are absolutely continuous with respect to the Lebesgue measure on $[0,T]\times[0,1]$. In the following, we write $\lambda(\cdot,\cdot)$ for the corresponding density.

\begin{lemma}
	\label{mapContLem}
	%CHECK.use uniformness
	%CHECK.approximating measure can be absolutely continuous, pure point, singular
	The function $\Phi$ is continuous at $\lambda(\cdot,\cdot)$.
\end{lemma}


As a first step in the proof of Lemma~\ref{mapContLem}, we provide bounds for the deviations of the increments 
$$(\va_{t_2}-\va_{t_2}^{(n)})-(\va_{t_1}-\va_{t_1}^{(n)}),\qquad0\le t_1\le t_2\le T$$

\begin{lemma}
	\label{incrLowLem}
	%CHECK.use monotonicity
	If $0\le t_1\le t_2\le T$, then
	\begin{align*}
		|\va'_{t_2}-\va_{t_2}|-|\va'_{t_1}-\va_{t_1}|&\le\Lambda'([t_1,t_2]\times[1-\va_{t_2},1-\va_{t_1}])+\sup_{t\in[t_1,t_2]}\Lambda'(\{t\},[0,1])\\
						      &\phantom{\ge}+|\int_{(t_1,t_2]}(\Lambda'-\Lambda)(\d s,[0,1-\va_s])|
	\end{align*}
\end{lemma}
\begin{proof}
	%CHECK.\le and \ge
	%CHECK.\va_t continuous
	%CHECK.degenerate t1',t2'
	As preliminary observation, we note that 
	\begin{align}
		\label{tzEq}
		\begin{split}
			\va'_{t_2}-\va_{t_2}&=\va'_{t_1}-\va_{t_2}+\int_{(t_1,t_2]}\Lambda'(\d s,[0,1-\va'_{s-}])\\
					    &=\va'_{t_1}-\va_{t_1}+\int_{(t_1,t_2]}\Lambda'(\d s,[0,1-\va'_{s-}])-\Lambda'(\d s,[0,1-\va_s])\\
	 &\phantom{=}+\int_{(t_1,t_2]}(\Lambda'-\Lambda)(\d s,[0,1-\va_s]).
		\end{split}
	\end{align}

	First, we provide a lower bound for $\va'_{t_2}-\va_{t_2}$. Without loss of generality, we may assume that $\va'_{t_2}<\va_{t_2}$. Then, by monotonicity,
	\begin{align*}
		\int_{(t_1,t_2]}\Lambda'(\d s,[0,1-\va'_{s-}])-\Lambda'(\d s,[0,1-\va_{s-}])&\ge\int_{(t_1,t_2]}\Lambda'(\d s,[0,1-\va_{t_2}])-\Lambda'(\d s,[0,1-\va_{s-}])\\
									      &\ge-\Lambda'([t_1,t_2]\times[1-\va_{t_2},1-\va_{t_1}]).
	\end{align*}
	Second, we provide an upper bound for $\va'_{t_2}-\va_{t_2}$. 
	Let $t_1^*\in[t_1,t_2]$ denote the infimum of all times $t\ge t_1$ such that $\va'_{t}\ge\va_{t_1}$. Similarly, we let $t_2^*\in[t_1,t_2]$ denote the 
	supremum of all times $t\le t_2$ such that $\va'_t\le\va_{t_2}$. Then, by monotonicity,
	\begin{align*}
		\int_{(t_1,t_2]}\Lambda'(\d s,[0,1-\va'_{s-}])-\Lambda'(\d s,[0,1-\va_s]&\le\int_{(t_1,t_2^*]}\Lambda'(\d s,[0,1-\va'_{s-}])-\Lambda'(\d s,[0,1-\va_{s-}])\\
											&=\int_{(t_1,t_1^*]}\Lambda'(\d s,[0,1-\va'_{s-}])-\Lambda'(\d s,[0,1-\va_{s-}])\\
			 &\phantom{=}+\int_{(t_1^*,t_2^*]}\Lambda'(\d s,[0,1-\va'_{s-}])-\Lambda'(\d s,[0,1-\va_{s-}]).
	\end{align*}
	For the first summand, we note that if $t_1^*>t_1$, then
	\begin{align*}
		\va'_{t_1}-\va_{t_1}+\int_{(t_1,t_1^*]}\Lambda'(\d s,[0,1-\va'_{s-}])\le \Lambda'(\{t_1^*\}\times[0,1])\le |\va_{t_1}-\va'_{t_1}|+\Lambda'(\{t_1^*\}\times[0,1]).
	\end{align*}
	When leaving out the intermediate step, this inequality certainly remains valid also if $t_1^*=t_1$. Moreover, by the definition of $t_1^*,t_2^*$, we may bound the second summand by
	\begin{align*}
		\int_{(t_1^*,t_2^*]}\Lambda'(\d s,[0,1-\va'_{s-}])-\Lambda'(\d s,[0,1-\va_{s-}])\le\Lambda'([t_1,t_2]\times[1-\va_{t_2},1-\va_{t_1}]).
	\end{align*}
	Inserting these bounds into~\eqref{tzEq} completes the proof.
\end{proof}
Using Lemma~\ref{incrLowLem}, we can now prove the continuity of $\Phi$.

\begin{proof}[Proof of Lemma~\ref{mapContLem}.]
	%CHECK.use Lemma incrLowLem
	%CHECK.use absolute continuity
	Let $\mc{Z}=\{t_1,\ldots,t_n\}$ be a partition of the interval $[0,T]$. Then, applying Lemma~\ref{incrLowLem} repeatedly gives 
	$$|\va_T-\va^{(n)}_T|\le\sum_{t_i\in\mc{Z}}\Lambda([t_i,t_{i+1}]\times[1-\va_{t_{i+1}},1-\va_{t_i}])+\varepsilon,$$
	provided that $n\ge1$ is sufficiently large. By choosing the partition sufficiently fine, the first summand is smaller than $\varepsilon$ by absolute continuity of $\Lambda$.
\end{proof}

